Distributed Differential Privacy in Multi-Armed Bandits

We consider the standard $K$-armed bandit problem under a distributed trust model of differential privacy (DP), which enables to guarantee privacy without a trustworthy server. Under this trust model, previous work largely focus on achieving privacy using a shuffle protocol, where a batch of users data are randomly permuted before sending to a central server. This protocol achieves ($\epsilon,\delta$) or approximate-DP guarantee by sacrificing an additional additive $O\!\left(\!\frac{K\log T\sqrt{\log(1/\delta)}}{\epsilon}\!\right)\!$ cost in $T$-step cumulative regret. In contrast, the optimal privacy cost for achieving a stronger ($\epsilon,0$) or pure-DP guarantee under the widely used central trust model is only $\Theta\!\left(\!\frac{K\log T}{\epsilon}\!\right)\!$, where, however, a trusted server is required. In this work, we aim to obtain a pure-DP guarantee under distributed trust model while sacrificing no more regret than that under central trust model. We achieve this by designing a generic bandit algorithm based on successive arm elimination, where privacy is guaranteed by corrupting rewards with an equivalent discrete Laplace noise ensured by a secure computation protocol. We also show that our algorithm, when instantiated with Skellam noise and the secure protocol, ensures \emph{R\'{e}nyi differential privacy} -- a stronger notion than approximate DP -- under distributed trust model with a privacy cost of $O\!\left(\!\frac{K\sqrt{\log T}}{\epsilon}\!\right)\!$.

==> MAB with SecAgg (arxiv)/content.tex <==
\section{Introduction}
The multi-armed bandit (MAB)~\cite{berry1985bandit} problem provides a simple but powerful framework for sequential decision-making under uncertainty with bandit feedback, which has attracted a wide range of practical applications such as online advertising \cite{abe2003reinforcement}, product recommendations \cite{li2010contextual}, clinical trials \cite{tewari2017ads}, to name a few. Along with its broad applicability, however, there is an increasing concern of privacy risk in MAB due to its intrinsic dependence on users' feedback, which could leak users' sensitive information~\cite{pan2019you}.
% has the potential of leaking users' sensitive information. 

% To illustrate this, let us consider a simplified music app that uses MAB algorithm to recommend music to its users. Suppose a Latin girl named Alice recently downloads the app and likes many Latin music. As a result of MAB recommendations, another user named Bob may recognize that this music app starts to recommend Latin music. If Bob is an adversary who happens to have the auxiliary information that Alice is the only most recent new user of this app, then Bob's belief that Alice is Latin will increase, which leads to a privacy risk of Alice's ethical information. Although our illustrating example seems simple, a similar privacy leakage has been observed in more advanced and practical online learning scenarios~\cite{pan2019you}. \sayak{We might not need this example and can direct jump on by stating that we need pure DP guarantee in distributed protocol. I can work on this.}

To alleviate the above concern, the notion of \emph{differential privacy}, introduced by \cite{dwork2006calibrating} in the field of computer science theory, has recently been adopted to design privacy-preserving bandit algorithms (see, e.g., \cite{mishra2015nearly,tossou2016algorithms,shariff2018differentially}). Differential privacy (DP) provides a principled way to mathematically prove privacy guarantees against adversaries with arbitrary auxiliary information about users. To achieve this, a differentially private bandit algorithm typically relies on a well-tuned random noise to obscure each user's contribution to the output, depending on privacy levels $\epsilon, \delta$ -- smaller values lead to stronger protection but also suffer worse utility (i.e., regret). For example, the central server of a recommendation system can use random noise to perturb its statistics on each item after receiving feedback (i.e., clicks/ratings) from users. This is often termed as \emph{central model}~\cite{dwork2014algorithmic}, since the central server has the trust of its users and hence has a direct access to their raw data. Under this model, an optimal private MAB algorithm with a pure DP guarantee (i.e., when $\delta = 0$) is proposed in~\cite{sajed2019optimal}, which only incurs an \emph{additive} $O\left(\frac{K\log T}{\epsilon}\right)$ term in the cumulative regret compared to the standard setting when privacy is not sought after \cite{auer2002using}. 
% various private MAB algorithms have been proposed [] and the one in [] achieves pure DP (i.e., $\delta = 0$) while only incurring an additional additive term in the utility (i.e., regret) compared to the non-private one. This actually matches the corresponding regret lower bound order-wise (see Table~\ref{tab-summary}). 
However, this high trust model is not always feasible in practice since users may not be willing to share their raw data directly to the server. This motivates to employ a \emph{local model}~\cite{kasiviswanathan2011can} of trust, where DP is achieved without a trusted server as each user perturbs her data prior to sharing with the server. This ensures a stronger privacy protection, but leads to a high cost in utility due to large aggregated noise from all users. As shown in~\cite{ren2020multi}, under the local model, private MAB algorithms  have to incur a \emph{multiplicative} $1/\epsilon^2$ factor in the regret rather than the additive one in the central model. 




In attempts to recover the same utility of central model while without a trustworthy server like the local model, an intermediate DP trust model called \emph{distributed model} has gained an increasing interest, especially in the context of (federated) supervised learning~\cite{kairouz2021advances,agarwal2021skellam,kairouz2021distributed,girgis2021shuffled,lowy2021private}. Under this model, each user first perturbs her data via a local randomizer, and then sends the randomized data to a \emph{secure} computation function. This secure function can be leveraged to guarantee privacy through aggregated noise from distributed users.
% The ``secure'' nature of this function guarantees that its output to the server is differentially private thanks to the aggregated noise from distributed users
% \xingyu{this part is not rigorous, security does not necessarily mean privacy. In particular, security only guarantees the server cannot see any particular user's data or guess which data belongs to a particular user, but this does not lead to DP (DP only comes from the added noise). That is, no matter how secure it is, it does not provide any DP if each user did not add noise. The correct way is to say something like: this secure function can be leveraged to guarantee privacy through distributed noise at each user... }. 
There are two popular secure computation functions: \emph{secure aggregation} (SecAgg)~\cite{bonawitz2017practical} and \emph{secure shuffling}~\cite{bittau2017prochlo}. The former often relies on cryptographic primitives to securely aggregate users' data so that the server only learns the aggregated result, while the latter securely shuffle users' messages to hide their source. To the best of our knowledge, distributed DP model is far less studied in online learning as compared to supervised learning, with only known results for standard $K$-armed bandits in~\cite{tenenbaum2021differentially} where only secure shuffling is adopted.
Despite being pioneer work, the results obtained in this paper have several limitations: (i) The privacy guarantee is obtained only for approximate DP ($\delta > 0$) -- a stronger pure DP ($\delta = 0$) guarantee is not achieved; (ii) The cost of privacy is a multiplicative $\sqrt{\log(1/\delta)}$ factor away from that of central model, leading to a higher regret bound; (iii) The secure protocol works only for binary rewards (or communication intensive for real rewards).\footnote{For more general linear bandits under distributed DP, see ~\cite{chowdhury2022shuffle,garcelon2022privacy}, which also have similar limitations.}  All of these lead to the following primary question:
\begin{center}
   \emph{Is there a communication-efficient MAB algorithm that satisfies pure DP in the distributed model while attaining the same regret bound as in the central model?  } 
\end{center}

% Furthermore, in addition to pure DP, it is of natural interest to offer a slightly weaker privacy guarantee (that is still stronger than approximate DP) in the interest of gaining improvement in utility. One such notion of privacy is \emph{R\'{e}nyi differential privacy} (RDP)~\cite{mironov2017renyi}, which, in addition to offering a gain in utility, also provides a tighter privacy accounting for composition compared to approximate DP. This is particularly useful for bandit algorithms, when users participate in multiple rounds, necessitating the need for privacy composition. This motivates us to study the question: \emph{Is there a bandit algorithm that guarantee RDP (with a better regret bound than pure-DP) in the distributed trust model?}
% \sayak{Needs more work - will do.}

\begin{table}[t]
  \caption{Best-known performance of private MAB under different privacy models ($K=$ number of arms, $T=$ time horizon, $\Delta_a$= reward gap of arm $a$ w.r.t. best arm, $\epsilon,\delta,\alpha=$ privacy parameters)}
  \label{tab-summary}
  \centering
  \begin{tabular}{lll}
    \toprule
    % \multicolumn{2}{c}{Part}                   \\
    % \cmidrule(r){1-2}
    Trust Model     & Privacy Guarantee     & Best-Known Regret Bounds \\
    \midrule
    Central & $(\epsilon,0)$-DP  & $\Theta\left(\sum_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a} +\frac{K\log T}{\epsilon}\right)$~\cite{sajed2019optimal,shariff2018differentially}     \\
    %Central     & $(\epsilon,\delta)$-DP  & $O\left(\sum_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a} +\frac{K}{\epsilon}\right)$~\cite{tossou2016algorithms}\\
    Local     & $(\epsilon,0)$-DP      & $\Theta\left(\frac{1}{\epsilon^2}\sum_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a}\right)$~\cite{ren2020multi}  \\
     %Local     & $(\epsilon,\delta)$-DP      & $O\left(\frac{\log(1/\delta)}{\epsilon^2}\sum_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a}\right)$~\cite{zheng2020locally}  \\
    Distributed      & $(\epsilon,\delta)$-DP      & $O\left(\sum_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a} +\frac{K\log T\sqrt{\log(1/\delta)}}{\epsilon}\right)$~\cite{tenenbaum2021differentially}  \\
     \cellcolor{LightCyan}Distributed     & \cellcolor{LightCyan}$(\epsilon,0)$-DP      & \cellcolor{LightCyan}$O\left(\sum_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a} +\frac{K\log T}{\epsilon}\right)$~(Thms.~\ref{thm:pure-SecAgg}~\ref{thm:pure-shuffle})   \\
      %\cellcolor{LightCyan}Distributed (via shuffling)     & \cellcolor{LightCyan}$(\epsilon,0)$-DP      & \cellcolor{LightCyan}$O\left(\sum_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a} +\frac{K\log T}{\epsilon}\right)$~(Thm.~\ref{thm:pure-shuffle})   \\
      \cellcolor{LightCyan}Distributed      & \cellcolor{LightCyan}$O(\alpha,\frac{\alpha \epsilon^2}{2})$-RDP      & \cellcolor{LightCyan}$O\left(\sum_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a} +\frac{K\sqrt{\log T}}{\epsilon}\right)$~(Thm.~\ref{thm:rdp-SecAgg})   \\
    \bottomrule
  \end{tabular}
  \vspace{-5mm}
\end{table}

% \textbf{Our contributions.} We answer this in the affirmative (see Table~\ref{tab-summary}) by overcoming several key challenges that arises in the distributed DP model for bandits. First, most known secure shuffling protocols only offer approximate DP for private sums. Second, SecAgg typically works only in the integer domain due to modular operation. This directly requires substantial changes to existing private MAB algorithms, including  data quantization, distributed discrete noise and modular summation arithmetic. Moreover, compared to supervised learning where typically a mean-square error bound on the noise is sufficient, private MAB requires a tight tail bound for the utility analysis, which becomes more challenging due to aforementioned changes and the constraints of communication in the distributed model. Finally, to guarantee RDP with discrete noise, one can no longer use continuous Gaussian mechanism and meanwhile binomial noise in~\cite{tenenbaum2021differentially} only provides approximate DP. 
% We take a systematic approach to address all the challenges, which is summarized 
% \begin{itemize}
%     \item We first propose a general algorithmic framework for private MAB in the distributed model building on a batch-based successive elimination algorithm. This algorithm relies on a template protocol $\cP_t = (\cR,\cS,\cA)$  tailored for discrete noise and modular operation,  which consists of a local randomizer $\cR$ at each user,  a generic secure computation function $\cS$ and an analyzer $\cA$ at the server. This template protocol not only enables us to achieve different privacy guarantees (e.g., pure DP/RDP) by tuning the noise in $\cR$, but allows for a unified analysis when using SecAgg and scure shuffling as the secure computation function $\cS$. 
%     \item We start with instantiating $\cR$ at each user with a proper P\'{o}lya random noise so that the total noise seen by the server is a discrete Laplace. With this choice, we show that pure DP can be attained in the distributed model with both SecAgg and secure shuffling. Moreover, the corresponding regret bound matches the one in the central model and the communication bits per user scale only logarithmicly with respect to participating users in each batch . 
%     \item We then consider achieving RDP in the distributed model by instantiating $\cR$ at each user with a Skellam random noise. Building on a novel concentration result on Skellam distribution, we show that RDP is also attainable in the distributed model.
%     \item Along the way...concentration for Skellam and central and local models with discrete noise...
% \end{itemize}


\textbf{Our contributions.} We answer this in the affirmative (see Table~\ref{tab-summary}) by overcoming several key challenges that arise in the distributed DP model for bandits. 
% First, most known secure shuffling protocols only offer approximate DP for private sums. 
First, although secure aggregation protocol offers a benefit in communication cost, it works only in the integer domain due to an inherent modular operation \cite{bonawitz2017practical}. This immediately requires substantial changes to existing private bandit algorithms, including data quantization, distributed \emph{discrete privacy noise} and modular summation arithmetic. Second, compared to supervised learning where typically a bound on the noise variance is sufficient to analyse utility, regret analysis of private bandits require a tight tail bound. This gets more challenging due to aforementioned requirements and communication constraints in the distributed model. 
% Finally, to guarantee RDP with discrete noise, one can no longer use continuous Gaussian mechanism and meanwhile binomial noise in~\cite{tenenbaum2021differentially} only provides approximate DP. 
We take a systematic approach to address these challenges, which is summarized below:

\textbf{1.} We propose a private bandit algorithm using a batch-variant of the successive arm elimination technique as a building block. We ensure distributed DP via a private protocol $\cP = (\cR,\cS,\cA)$ tailored to discrete noise and modular operation (see Algorithm~\ref{alg:SE}, \ref{alg:randomizer}, \ref{alg:analyzer}). It consists of a local randomizer $\cR$ at each user, a generic secure computation function $\cS$, and an analyzer $\cA$ at the server. This template protocol not only enables us to achieve different privacy guarantees by tuning the noise in $\cR$, but allows a unified analysis for different secure computation functions $\cS$ (i.e., both SecAgg and secure shuffling). 

\textbf{2.} To achieve pure DP guarantee, we instantiate $\cR$ at each user with an appropriate P\'{o}lya random noise so that the total noise seen by the server is a discrete Laplace. 
% With this choice, we show that pure DP can be attained in the distributed model with both SecAgg and secure shuffling. 
Using tail properties of discrete Laplace, we show that the cumulative regret of our algorithm matches the one in the central model, achieving the optimal rate under pure DP (see Theorem~\ref{thm:pure-SecAgg}, \ref{thm:pure-shuffle}). Moreover, the communication bits per-user scale only logarithmicaly with the number of participating users in each batch.

\textbf{3.} In addition to pure DP, it is of natural interest to offer a slightly weaker privacy guarantee (but, still stronger than approximate DP) in the hope of gaining improvement in utility. One such notion of privacy is \emph{R\'{e}nyi differential privacy} (RDP)~\cite{mironov2017renyi}, which, in addition to offering a gain in utility, also provides a tighter privacy accounting for composition compared to approximate DP. This is particularly useful for bandit algorithms, when users may participate in multiple rounds, necessitating the need for privacy composition. 
% This motivates us to study the question: \emph{Is there a bandit algorithm that guarantee RDP (with a better regret bound than pure-DP) in the distributed trust model?}
To this end, we obtain RDP in the distributed model by instantiating $\cR$ at each user with a Skellam random noise. Proving a novel tail-bound for Skellam distribution, we show that a tighter regret bound compared to pure DP can be achieved (see Theorem~\ref{thm:rdp-SecAgg}).

\textbf{4.} We numerically evaluate the regret performance of our algorithm under both DP and RDP guarantees, which corroborate our theoretical results.

\textbf{Related work.} We have covered the most relevant works. Please refer to Appendix~\ref{app:related} for other works.

% \xingyu{intro is nice:). Thanks Sayak!}

% \xingyu{BTW, where shall we put related work?}\sayak{No space and hence no need unless there is something very related stuff missing }
% RDP is also attainable in the distributed model. Along the way...concentration for Skellam and central and local models with discrete noise...

%\textbf{Related Work.} 

% \xingyu{This part is easy...I will first finish the conclusion remarks and we might need the simulation parts done by our next meeting so that we have another week to polish the whole paper:)}
% \sayak{Sure. Will put some. Sorry for the prolonged silence.}\xingyu{Great! no problem:) I have finished all the technical parts. BTW, UCB-type algorithm can indeed achieve optimal pure-DP regret bound, see conclusion remark section and appendix. }


% \xingyu{For the simulation: we need to consider real-valued reward to demonstrate the effectiveness of our data quantization scheme in $\cP_t$ (i.e., fix-point encoding, which is necessary for real-valued rewards). 
% More details are as follows:
% \begin{itemize}
%     \item Sajed's scheme (of course only continous noise)
%     \item Our SecAgg for pure DP with discrete Laplace
%     \item Our SecAgg for RDP via Skellam 
% \end{itemize}
% \sayak{I am getting exact same results for discreet laplace and skellam (using scale =1).}\xingyu{can we tune the skellam a little bit to show a slight advantage in regret? For example, how large is your choice of $s$ (scaling factor in the theorem) in the Skellam mechanism? For a larger scaling factor, we have a larger communication, but it also improves the regret}\sayak{Doing $s=10$, but same bound as DP.}\xingyu{can we try a larger $s$? since the message here is that Skellam possibly would improve the regret as stated in the theorem for a large enough $s$, i.e., $s \ge \sqrt{\log T}$.} \sayak{$T=10^7$ here. So, $s=10$ seems fine. However, will try with sat $s=100$?}\xingyu{Got it! Yes, try a larger one so that we can delivery the message:)}\sayak{Getting same bound for $s=1,10,100$}


% The above three are the minimum for the simulations I think. In addition to them, we can further consider
% \begin{itemize}
%     \item Local model (we can implement our version of local model with discrete noise rather than my previous paper, see Appendix~\ref{app:central-local})
%     \item UCB-type algorithm for pure DP via SecAgg, see Appendix~\ref{app:UCB}

% \end{itemize}
% Finally, the deadline is approaching and we only have one week for the main paper:)
% }


\section{Preliminaries}
In this section, we formally introduce the distributed differential privacy model in bandits. Before that we recall the learning paradigm in multi-armed bandits and basic differential privacy definitions. 

% \paragraph{Learning model and regret in MAB}
\textbf{Learning Model and Regret in MAB.}
At each time slot $t \in [T]:= \{1,\ldots, T\}$, the agent (e.g., recommender system) selects an arm $a \in [K]$ (e.g., an advertisement) and obtains an i.i.d reward $r_t$ from user $t$ (e.g., a rating indicating how much she likes it), which is sampled from a distribution over $[0,1]$ with mean given by $\mu_a$. Let $a^*:=\argmax_{a \in [K]}\mu_a$ be the arm with the highest mean and denote $\mu^*:= \mu_{a^*}$ for simplicity. Let $\Delta_a:= \mu^* - \mu_a$ be the gap of the expected reward between the optimal arm $a^*$ and any other arm $a$. Further, let $N_a(t)$ be the total number of times that arm $a$ has been played in the first $t$ rounds.
The goal of the agent is to maximize its total reward, or equivalently to minimize the cumulative expected
pseudo-regret, defined as
\begin{align*}
    \ex{\text{Reg}(T)} := T\cdot \mu^* - \ex{\sum\nolimits_{t=1}^T r_t} = \ex{\sum\nolimits_{a \in [K]} \Delta_a N_a(T)}.
\end{align*}
% \paragraph{Differential Privacy}
\textbf{Differential Privacy.}
% We first present necessary differential privacy notions used in this paper and will specify them in the setting of MAB under different trust models in the next section. 
% Note that in the context of MAB, the privacy concerns the rewards $\{r_t\}_{t \in [T]}$ received from users since these data could reveal sensitive information about users. 
% Let $\cD$ be the data universe, we say $D, D'\in \cD^n$ are neighboring datasets if they only differ in a single element. With this, we have the following standard definition of differential privacy~\cite{dwork2006calibrating}.
% We first present necessary differential privacy notions used in this paper and will specify them in the setting of MAB under different trust models in the next section.
Let $\cD = [0,1]$ be the data universe, and $n\in \Nat$ be the number of \emph{unique} users. we say $D, D'\in \cD^n$ are neighboring datasets if they only differ in 
one user's reward $D_i$ for some $i \in [n]$. With this, we have the following standard definition of differential privacy~\cite{dwork2006calibrating}.

% a single element. .
% In the context of MAB, the private data is the reward received from each user. That is, we have $\cD = [0,1]$ and $D,D' \in \cD^n$ are two neighboring datasets consisting of $n$ \emph{unique} users' rewards, which only differ in one user's reward $D_i$ for some $i \in [n]$.

\begin{definition}[Differential Privacy]
\label{def:DP}
For $\epsilon,\delta >0$, a randomized mechanism $\cM$ satisfies $(\epsilon,\delta)$-DP if for all neighboring datasets $D,D'$ and all events $\cE$ in the range of $\cM$, we have 
\begin{align*}
    \prob{\cM(D) \in \cE} \le e^{\epsilon}\cdot \prob{\cM(D') \in \cE} + \delta.
\end{align*}
\end{definition}

The special case of $(\epsilon,0)$-DP is often referred to as \emph{pure differential privacy}, whereas, for $\delta>0$, $(\epsilon,\delta)$-DP is referred to as \emph{approximate differential privacy}.
% We will also make use of R\'{e}nyi differential privacy (RDP)~\cite{mironov2017renyi} 
% and concentrated differential privacy (CDP)~\cite{bun2016concentrated}, which allow for a tighter composition compared to working with approximate-DP directly.
We also consider a related notion of privacy called R\'{e}nyi differential privacy (RDP)~\cite{mironov2017renyi}, which allow for a tighter composition compared to approximate differential privacy.
\begin{definition}[R\'{e}nyi Differential Privacy]
\label{def:RDP}
For $\alpha > 1$, a randomized mechanism $\cM$ satisfies $(\alpha, \epsilon(\alpha))$-RDP if for all neighboring datasets $D,D'$, we have $D_{\alpha}(\cM(D),\cM(D')) \le \epsilon(\alpha)$, where $D_{\alpha}(P,Q)$ is the R\'{e}nyi divergence (of order $\alpha$) of the distribution $P$ from the distribution $Q$, and is given by 
\begin{align*}
    D_{\alpha}(P, Q):= \frac{1}{\alpha-1}\log\left(\mathbb{E}_{x\sim Q}\left[ \left(\frac{P(x)}{Q(x)}\right)^\alpha \right]\right).
\end{align*}
\end{definition}

% \begin{definition}[Concentrated Differential Privacy]
% \label{def:CDP}
% A randomized mechanism $\cM$ satisfies $\frac{1}{2}\epsilon^2$-CDP if for all neighboring datasets $D,D'$ and all $\alpha \in (1,\infty)$, we have $D_{\alpha}(\cM(D),\cM(D')) \le \frac{1}{2}\epsilon^2 \alpha$.
% \end{definition}
% From the definitions above, we can see that $(\epsilon,0)$-DP is equivalent to $(\infty,\epsilon)$-RDP.
% and $\frac{1}{2}\epsilon^2$-CDP is equivalent to satisfying $(\alpha,\frac{1}{2}\epsilon^2\alpha)$-RDP simultaneously for all $\alpha \in (1,\infty)$. 

% Moreover, we have the following conversion lemma~\cite{balle2020hypothesis,canonne2020discrete,asoodeh2020better}.
% \begin{lemma}[Conversion Lemma]
% \label{lem:conversion}
% If $\cM$ satisfies $(\alpha, \epsilon(\alpha))$-RDP, then for any $\delta \in (0,1)$, $\cM$ satisfies $(\epsilon,\delta)$-DP where 
% \begin{align*}
%     \epsilon = \inf_{\alpha>1} \epsilon(\alpha) + \frac{\log(1/(\alpha \delta))}{\alpha - 1} + \log(1-1/\alpha).
% \end{align*}
% % If $\cM$ satisfies $\frac{1}{2}\epsilon^2$-CDP, then for for any $\delta \in (0,1)$, $\cM$ satisfies $(\epsilon',\delta)$-DP where 
% % \begin{align*}
% %     \epsilon' = \inf_{\alpha>1} \frac{1}{2}\epsilon^2 \alpha + \frac{\log(1/(\alpha \delta))}{\alpha - 1} + \log(1-1/\alpha) \le \epsilon\cdot \left(\sqrt{2\log(1/\delta)} +\epsilon/2\right).
% % \end{align*}
% Moreover, if $\cM$ satisfies $(\epsilon,0)$-DP, then it satisfies $(\alpha,\frac{1}{2}\epsilon^2\alpha)$-RDP simultaneously for all $\alpha \in (1,\infty)$.
% \end{lemma}
% \begin{remark}
% As with standard DP, RDP also satisfies post-processing property~\cite{mironov2017renyi}. 
% \end{remark}

% \subsection{Privacy Model in MAB}
% In the following, we will formally introduce the central, local and distributed DP models in MAB. In particular, we will present them in a unified way, which not only helps to highlight the key difference among them, but provides a modular decomposition for designing private bandit learning protocols under different trust models, which will be leveraged in later sections.


% In the context of MAB, the private data is the reward received from each user. That is, we have $\cD = [0,1]$ and $D,D' \in \cD^n$ are two neighboring datasets consisting of $n$ \emph{unique} users' rewards, which only differ in one user's reward $D_i$ for some $i \in [n]$. We consider a general bandit learning protocol $\cP = (\cR,\cS,\cA)$ that consists of three parts: (i) a (local) randomizer $\cR$ at each user's side, (ii) an intermediate secure protocol $\cS$ (iii) an analyzer $\cA$ at the central server. Each user $i$ first applies randomizer on its raw reward $D_i$ and then the randomized data $\cR(D_i)$ will go through the intermediate protocol  $\cS$ (e.g., SecAgg or shuffling). Finally, the server utilizes an analyzer $\cA$ to compute the output (i.e., action) using received messages from $\cS$.

% \paragraph{Central and Local Differential Privacy}
% We start with the central model, in which the central server is trusted and hence users' rewards are directly collected at the server, i.e., both $\cR$ and $\cS$ in $\cP$ are simply identity mappings. 

% In the central model, the privacy burden is at the analyzer $\cA$ which needs to inject necessary random noise to achieve privacy, i.e., an adversary observing the prescribed actions cannot infer too much information about any particular user. Formally, we have the following definition.

% \begin{definition}[Central DP Model]
% Under the central model, $\cP = (\cR,\cS,\cA)$ has identity mappings for both $\cR$ and $\cS$. $\cP$ is said to satisfy central-DP (or RDP) if the mechanism $\cA$ satisfies Definition~\ref{def:DP} (or Definitions~\ref{def:RDP}). More specifically, $D, D'$ are neighboring datasets of $T$ users' rewards.
% \end{definition}



% The central model has been extensively utilized in designing private MAB algorithms []. In particular, the developed algorithm in~\cite{sajed2019optimal} achieves the optimal regret bound that matches the lower bound for the central model in~\cite{shariff2018differentially} (see Table). 

% However, the assumption of a trusted server in the central model may be too strong in practice. This directly motivates the local model, under which privacy is guaranteed without a trusted server. This is achieved by privatizing each user's raw data via the local randomizer $\cR$ (with $\cS$ being an identity mapping) and hence by the post-processing of DP (or RDP), the same level of privacy is preserved for the whole protocol $\cP$. More specifically, we have the following definition.

% On the other hand, in the local model, each user's data has already been privatized by local $\cR$.
% \begin{definition}[Local DP Model]
% Under the local model, $\cP = (\cR,\cS,\cA)$ has an identity mapping for $\cS$. $\cP$ is said to satisfy local-DP (or RDP) if the mechanism $\cR$ satisfies Definition~\ref{def:DP} (or Definitions~\ref{def:RDP}). Here, the neighboring datasets are the local rewards  $D_i, D_i^{\prime} \in \cD$ for any $i \in [T]$.
% \end{definition}

% \paragraph{Distributed Differential Privacy}
\textbf{Distributed Differential Privacy.}
% While the local model can warrant privacy protection without a trusted server, the utility performance (i.e., regret) downgrades substantially due to larger amount of noise added compared to the central model (see Table). Thus, there is a natural need for a trust model of differential privacy that can interpolate between the central model and local model. This leads to the recently proposed \emph{distributed DP model}, which aims to recover the utility of central model while without trusting the central server.
% In the following, we will formally introduce the central, local and distributed DP models in MAB. In particular, we will present them in a unified way, which not only helps to highlight the key difference among them, but provides a modular decomposition for designing private bandit learning protocols under different trust models, which will be leveraged in later sections.
A distributed bandit learning protocol $\cP = (\cR,\cS,\cA)$ consists of three parts: (i) a (local) randomizer $\cR$ at each user's side, (ii) an intermediate secure protocol $\cS$, and (iii) an analyzer $\cA$ at the central server. Each user $i$ first locally apply the randomizer $\cR$ on its raw data (i.e., reward) $D_i$, and sends the randomized data to a secure computation protocol $\cS$ (e.g., secure aggregation or shuffling). This intermediate secure protocol $\cS$ takes a batch of users' randomized data and generates inputs to the  central server, which utilizes an analyzer $\cA$ to compute the output (e.g., action) using received messages from $\cS$.

 






The secure computation protocol $\cS$ has two main variations: \emph{secure shuffling} and \emph{secure aggregation}. Both of them essentially work with a batch of users' randomized data and guarantee that the central server cannot infer any individual's data while the total noise in the inputs to the analyzer provides a high privacy level.
% (see Appendix~\ref{app:secAggshuffle} for more discussions). 
To adapt both into our MAB protocol, it is natural to divide participating users into batches. For each batch $b \in [B]$ with $n_b$ users, the outputs of $\cS$ is given by $ \cS \circ \cR^{n_b}(D):=\cS(\cR(D_1),\ldots, \cR(D_{n_b}))$. The goal is to guarantee that the the view of all $B$ batches' outputs satisfy DP. To this end, we define a (composite) mechanism 
\begin{align*}
%\label{def:comp_mech}
    \cM_{\cP}=(\cS \circ \cR^{n_1},\ldots,\cS \circ \cR^{n_B}),
\end{align*}
where each individual mechanism $\cS \circ \cR^{n_b}$ operates on $n_b$ users' rewards, i.e., on a dataset from $\cD^{n_b}$. With this notation, we have the following definition of distributed differential privacy.
\begin{definition}[Distributed DP]
A protocol $\cP = (\cR,\cS,\cA)$ is said to satisfy DP (or RDP) in the distributed model if the mechanism $\cM_{\cP}$ satisfies Definition~\ref{def:DP} (or Definition~\ref{def:RDP}).
\end{definition}


In the central DP model, the privacy burden lies with a central server (in particular, analyzer $\cA$), which needs to inject necessary random noise to achieve privacy. On the other hand, in the local DP model, each user's data is privatized by local randomizer $\cR$.
% i.e., an adversary observing the prescribed actions cannot infer too much information about any particular user. 
% On the other hand, in the local model, each user's data has already been privatized by local $\cR$.
In contrast, in the distributed DP model, privacy without a trusted central server is achieved by ensuring that the inputs to the analyzer $\cA$ already satisfy differential privacy. Specifically, by properly designing the intermediate protocol $\cS$ and the noise level in the randomizer $\cR$, one can ensure that the final added noise in the aggregated data over a batch of users matches the noise that would have otherwise been added in the central model by the trusted server.
% (i.e., a large variance/low $\epsilon$). 
Through this, distributed DP model provides the possibility to achieve the same level of utility as the central model without a trustworthy central server.

% Roughly speaking, under the local model, privacy is achieved without a trusted server since the data that leaves each user's side has already been privatized by its local randomizer $\cR$. By the post-processing of DP (or RDP/CDP), the same privacy guarantee is maintained afterwards. Therefore, local model provides a strictly stronger privacy guarantee 

% \begin{algorithm}[tb]
%   \caption{Batch-Based  Successive Elimination}
%   \label{alg:SE}
% \begin{algorithmic}[1]
%   \STATE {\bfseries Parameters:} Number of arms $K$, Time horizon $T$, Privacy protocol $\cP \!=\! (\cR, \cS, \cA)$, privacy level $\epsilon > 0$, Confidence radii $\{\beta(b)\}_{b\ge 1}$.
%   \STATE {\bfseries Initialize:} Batch counter $b\!=\!1$, Estimate $\hat{\mu}_a(1) \!=\! 0,~\forall a$, Active set of arms $\Phi(b) \!=\! \{1,\ldots, K\}$
%  \FOR{batch $b\!=\!1, 2,\dots$}
% %   \STATE The local algorithm is updated with $\hat{\theta}_m$ and $V_m$ 
%     \STATE Set batch size $l(b) \!=\! 2^b$ 
%     \FOR{each active $a \in \Phi(b)$}
%       % \STATE Reset estimate $\hat{\mu}_a(b) \!=\!0$
%         \FOR{each new user $i$ from 1 to $l(b)$}
%             \STATE Pull arm $a$ and generate reward $r_{a}^i(b)$
%             \STATE Send randomized data $y_a^i(b) \!=\! \cR(r_a^i(b))$ to secure computation protocol $\cS$ \textcolor{gray}{//  randomizer}
%             \STATE If total number of pulls reaches $T$, \textbf{exit}
%         \ENDFOR
%          \STATE Send messages $\hat{y}_a(b)\!=\! \cS(\{{y}_a^i(b)\}_{1\le i\le l(b)})$ to the analyzer \textcolor{gray}{// secure computation protocol}
%         %   \STATE Post-processing messages ${y}_a(b)\!=\!\texttt{POST}(\hat{y}_a(b))$, if necessary
%           \STATE Compute the sum of rewards $R_a(b)\!=\!\cA(\hat{y}_a(b))$ \COMMENT{analyzer}
%           \STATE Compute current estimate $\hat{\mu}_a(b) \!=\! R_a(b) / l(b)$
%           \STATE Compute confidence bounds: $\text{UCB}_a(b)\!=\! \hat{\mu}_a(b) \!+\! \beta(b)$ and $\text{LCB}_a(b)\!=\! \hat{\mu}_a(b) \!-\! \beta(b)$
%     \ENDFOR
%     %\STATE Eliminate all arms $a \in \Phi$ such that $\text{UCB}_a(b) \!<\! \max_{a'\in \Phi}\text{LCB}_a(b)$
%     \STATE Update active set of arms: $\Phi(b\!+\!1)\!=\!\lbrace a \!\in\! \Phi(b): \text{UCB}_a(b) \!\ge \! \max_{a'\in \Phi(b)}\text{LCB}_{a'}(b) \rbrace $
%   \ENDFOR
% \end{algorithmic}
% \end{algorithm}


\section{A Generic Algorithm for Private Bandits}
 In this section, we propose a generic algorithmic framework for multi-armed bandits under the distributed privacy model. 
%  We build on the celebrated technique of successive arm elimination \sayak{cite even dar, Manor, Kalyankrishnan,..} that operates on top of a generic distributed DP protocol $\cP$, which is implemented using \emph{discrete} privacy noise. This protocol will be instantiated in later sections to obtain specific privacy and regret guarantees.

% We call it a meta algorithm because it only relies on a black-box protocol $\cP$, which will be instantiated in later sections under different trust models.

\subsection{Batch-Based Successive Elimination Algorithm}
Our generic algorithm (Algorithm~\ref{alg:SE}) builds upon the classic idea of successive arm elimination \cite{even2006action} with the additional incorporation of batches and a black-box protocol $\cP=(\cR,\cS,\cA)$ to achieve distributed differential privacy. More specifically, it divides the time horizon $T$ into batches of exponentially increasing size and eliminates sub-optimal arms successively. 
% For each batch, it doubles the batch size and then calculates the new mean estimates for each active arm. 
To this end, for each active arm $a$ at batch $b$, it first prescribes arm $a$ to a \emph{batch} of $l(b)$ new users.\footnote{In contrast, the classic successive elimination algorithm prescribes each arm to a single user.} After pulling the prescribed action $a$, each user applies the local randomizer $\cR$ to her reward and sends the randomized reward to the intermediary function $\cS$, which runs a secure protocol (e.g., secure aggregation or secure shuffling) over the total $l(b) $ number of randomized rewards. Then, upon receiving the outputs of $\cS$, the server applies the analyzer $\cA$ to compute the the sum of rewards for batch $b$ when pulling arm $a$, which gives the new mean estimate $\hat\mu_a(b)$ of arm $a$ after being divided by the total pulls $l(b)$. Then, upper and lower confidence bounds, $\text{UCB}_a(b)$ and $\text{LCB}_a(b)$, respectively, are computed around the mean estimate $\hat \mu_a(b)$ with a properly chosen confidence width $\beta(b)$. Finally, after the iteration over all active arms in batch $b$ (denoted by the set $\Phi(b)$), it adopts the standard arm elimination criterion to remove all obviously sub-optimal arms, i.e., it removes an arm $a$ from $\Phi(b)$ if $\text{UCB}_a(b)$ falls below $\text{LCB}_{a'}(b)$ of any other arm $a' \in \Phi(b)$. It now remains to design a distributed DP protocol $\cP$, which will be explored at length in the next section.

% This new mean estimate directly leads to new upper confidence bound (UCB) and lower confidence bound (LCB) over the true mean $\mu_a$. 
% Finally, after the iteration over all active arms in batch $b$, it adopts the standard arm elimination criterion to remove all obviously sub-optimal arms.

% One nice feature of our generic algorithm is its flexibility. In particular, it provides an algorithmic framework for designing private MAB algorithms under different trust models. To see this, one can easily design a private MAB algorithm under the central model by choosing $\cR$ and $\cS$ as identity mappings while $\cA$ being standard DP mechanisms (e.g., Laplace or Gaussian). On the other hand, an LDP MAB algorithm is obtained by  directly instantiating $\cR$ as standard DP algorithms while both $\cS$ and $\cA$ being identity mappings. More importantly, it also offers the flexibility to design  MAB algorithms under distributed DP in a unified way, which will be explored at length in the next section.




\subsection{Distributed DP Protocol via Discrete Privacy Noise}
In this section, inspired by~\cite{balle2020private,cheu2021pure}, we provide a general template protocol $\cP$ for the distributed DP model, which rely only on discrete privacy noise. The motivation behind using discrete noise is three-fold: (i) Practical secure aggregation (SecAgg) functions work only on the integer domain~\cite{bonawitz2017practical}; (ii) A real-value noise is often difficult to encode on finite computers in practice~\cite{canonne2020discrete,kairouz2021distributed} and a naive use of finite precision approximation may lead to a possible failure
of privacy protection~\cite{mironov2012significance};  (iii) Discrete noise enables communication via bits rather than real numbers, hence reducing communication overheads.
The detail of our template protocol $\cP = (\cR,\cS,\cA)$ for distributed DP model is as follows (see Algorithm~\ref{alg:randomizer},\ref{alg:analyzer} for pseudo-code). The local randomizer $\cR$ receives user's real-valued reward and encodes it as an integer via a fixed-point encoding with precision $g >0$ and randomized rounding. Then, it generates a discrete noise, which depends on the specific privacy-regret trade-off requirement (to be discussed later under specific mechanisms). Next, it adds the generated random noise into the encoded reward, modulo clips the sum and sends the final integer as input to $\cS$. Here, we leave $\cS$ as a black-box function that can be secure aggregation or shuffling, since both have advantages over the other (the engineering implementations of both functions are beyond the scope of this paper, see Appendix~\ref{app:secAggshuffle} for a brief discussion). Instead, a common high-level idea behind both techniques is to ensure that after receiving messages from $\cS$, the server cannot distinguish each individual's message. Finally, the job of the analyzer $\cA$ in our template protocol is to calculate the sum of rewards within a batch as accurately as possible. To this end, when $\cS$ is SecAgg, it directly corrects for possible underflow due to modular operation and bias due to encoding by $g$. Otherwise, when $\cS$ is shuffling, it first translates received messages (e.g., a collection of bits) into an integer by taking a modular sum over the multiset, and then corrects for the underflow. To sum it up, the end goal of our protocol $\cP$ is to ensure that it provides the required privacy protection while guaranteeing an output $z \approx \sum_{i=1}^{n} x_i$ with high probability, which is the key to our privacy and regret analysis in the following sections.

% In this section, we propose a general protocol $\cP = (\cR,\cS,\cA)$ in Algorithm~\ref{alg:SE} that only uses discrete private noise. In particular, we keep it as general as possible so that it is compatible with any discrete noise. In the later sections, we will instantiate it with specific private noise to balance between privacy and regret. 

\begin{algorithm}[tb]
  \caption{Batch-Based  Successive Elimination}
  \label{alg:SE}
\begin{algorithmic}[1]
  \STATE {\bfseries Parameters:} Number of arms $K$, Time horizon $T$, Privacy protocol $\cP \!=\! (\cR, \cS, \cA)$, privacy level $\epsilon > 0$, Confidence radii $\{\beta(b)\}_{b\ge 1}$.
  \STATE {\bfseries Initialize:} Batch counter $b\!=\!1$, Estimate $\hat{\mu}_a(1) \!=\! 0,~\forall a$, Active set of arms $\Phi(b) \!=\! \{1,\ldots, K\}$
 \FOR{batch $b\!=\!1, 2,\dots$}
%   \STATE The local algorithm is updated with $\hat{\theta}_m$ and $V_m$ 
    \STATE Set batch size $l(b) \!=\! 2^b$ 
    \FOR{each active arm $a \in \Phi(b)$}
      % \STATE Reset estimate $\hat{\mu}_a(b) \!=\!0$
        \FOR{each new user $i$ from 1 to $l(b)$}
            \STATE Pull arm $a$ and generate reward $r_{a}^i(b)$
            \STATE Send randomized data $y_a^i(b) \!=\! \cR(r_a^i(b))$ to secure computation protocol $\cS$ \textcolor{gray}{//  randomizer}
            \STATE If total number of pulls reaches $T$, \textbf{exit}
        \ENDFOR
         \STATE Send messages $\hat{y}_a(b)\!=\! \cS(\{{y}_a^i(b)\}_{1\le i\le l(b)})$ to the analyzer \textcolor{gray}{// secure computation protocol}
        %   \STATE Post-processing messages ${y}_a(b)\!=\!\texttt{POST}(\hat{y}_a(b))$, if necessary
          \STATE Compute the sum of rewards $R_a(b)\!=\!\cA(\hat{y}_a(b))$ \COMMENT{analyzer}
          \STATE Compute current estimate $\hat{\mu}_a(b) \!=\! R_a(b) / l(b)$
          \STATE Compute confidence bounds: $\text{UCB}_a(b)\!=\! \hat{\mu}_a(b) \!+\! \beta(b)$ and $\text{LCB}_a(b)\!=\! \hat{\mu}_a(b) \!-\! \beta(b)$
    \ENDFOR
    %\STATE Eliminate all arms $a \in \Phi$ such that $\text{UCB}_a(b) \!<\! \max_{a'\in \Phi}\text{LCB}_a(b)$
    \STATE Update active set of arms: $\Phi(b\!+\!1)\!=\!\lbrace a \!\in\! \Phi(b): \text{UCB}_a(b) \!\ge \! \max_{a'\in \Phi(b)}\text{LCB}_{a'}(b) \rbrace $
  \ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
  \caption{Local Randomizer $\cR$}
  \label{alg:randomizer}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} Each user data $x_i \in [0,1]$
%   \STATE {\bfseries Parameters:}  precision $g \in \mathbb{N}$, modulo $m \in \mathbb{N}$, batch size $n \in \mathbb{N}$, privacy parameter $\phi$
  \STATE {\bfseries Parameters:}  precision $g \in \mathbb{N}$, modulo $m \in \mathbb{N}$, batch size $n \in \mathbb{N}$, privacy level $\epsilon$
  \STATE Encode $x_i$ as $\hat{x}_i = \lfloor{x_i g}\rfloor + \textbf{Ber}(x_ig -\lfloor{x_i g}\rfloor)$
%   \STATE Generate discrete noise $\eta_i \sim \text{rand}(n,\phi)$ \textcolor{gray}{// a black-box random noise generator}
    \STATE Generate discrete noise $\eta_i$ (depending on $n,\epsilon,g$) \COMMENT{a black-box random noise generator}
  \STATE Add noise and modulo clip $y_i = (\hat{x}_i + \eta_i) \Mod m$
  \STATE {\bfseries Output:} $y_i$ \COMMENT{for secure computation protocol $\cS$}
\end{algorithmic}
\end{algorithm}
\vspace{-2mm}
\begin{algorithm}[!tb]
  \caption{Analyzer $\cA$}
%   \sayak{Can this be written as subroutine of Algo 1? Just to save some space. Also, is it possible to shift the gray texts to far right? I tried but failed...}
%   }\xingyu{I prefer to keep it as a building block. Let me try to put comments to right}
  \label{alg:analyzer}
\begin{algorithmic}[1]
    \STATE {\bfseries Input:} $\hat{y}$ (output of $\cS$) 
  \STATE {\bfseries Parameters:}  precision $g \in \mathbb{N}$, modulo $m \in \mathbb{N}$, batch size $n \in \mathbb{N}$, accuracy parameter $\tau \in \Real$
%   \STATE Let $y \in \mathbb{Z}_m$ be the result of first summing over $\hat{y}$ and then take modulo $m$ 
  \STATE \textbf{if} $\cS$ is Secure Shuffling \textbf{then}
\STATE $\quad$ set $y = (\sum \hat{y}) \Mod m  $ \COMMENT{$\hat{y}$ is a multiset for secure shuffling}
% \textcolor{gray}{// $\hat{y}$ is a vector for secure shuffling}
\STATE \textbf{else} set $y = \hat{y}$ \COMMENT{$\hat{y}$ is scalar for secure aggregation} 
% \textcolor{gray}{// $\hat{y}$ is scalar for secure aggregation}
%   \IF{$y > ng+\tau$}
%     \STATE $z = (y-m) / g$ \textcolor{gray}{// correction for underflow}
%   \ELSE
%     \STATE $z = y/g$
%   \ENDIF
\STATE \textbf{if} $y > ng+\tau$ \textbf{then}
\STATE $\quad$ set $z = (y-m) / g$ \COMMENT{correction for underflow}
\STATE \textbf{else} set $z = y/g$
  \STATE {\bfseries Output:} $z$
\end{algorithmic}
\end{algorithm}


% \begin{algorithm}[!tb]
%   \caption{Analyzer $\cA$}
%   \label{alg:analyzer}
% \begin{algorithmic}[1]
%     \STATE {\bfseries Input:} Integer $y \in \{0,1,\ldots,m-1\}$ \textcolor{gray}{// after post-processing}
%   \STATE {\bfseries Parameters:}  precision $g \in \mathbb{N}$, modulo $m \in \mathbb{N}$, batch size $n \in \mathbb{N}$, accuracy parameter $\tau$
%   \IF{$y > ng+\tau$}
%     \STATE $z = (y-m) / g$ \textcolor{gray}{// correction for underflow}
%   \ELSE
%     \STATE $z = y/g$
%   \ENDIF
%   \STATE {\bfseries Output:} $z$
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[h!]
% \caption{User procedure $\cA_{\text{user}}$}
% \label{alg:user}
% \DontPrintSemicolon
% \textbf{Input}: Data $x_i \in [0,1]$\;
% \textbf{Parameters}: precision $g \in \mathbb{N}$, modulo $m \in \mathbb{N}$, batch size $n \in \mathbb{N}$, privacy parameter $\phi$\;
% Encode $x_i$ as $\hat{x}_i = \lfloor{x_i g}\rfloor + \textbf{Ber}(x_ig -\lfloor{x_i g}\rfloor)$\;
% Generate noise $\eta_i = \cR(n,\phi)$ \textcolor{gray}{// a black-box random noise generator}\; 
% Add noise and modulo clip $y_i = \hat{x}_i + \eta_i \Mod m$\;
% \textbf{Output}: $y_i$ for the SecAgg protocol\;
% \end{algorithm}


% \begin{algorithm}[h!]
% \caption{Server procedure $\cA_{\text{server}}$}
% \label{alg:server}
% \DontPrintSemicolon
% \textbf{Input}: Integer $y \in \{0,1,\ldots, m-1\}$ \textcolor{gray}{// $y = \sum_i y_i \Mod m$ via SecAgg protocol} \;
% \textbf{Parameters}: precision $g \in \mathbb{N}$, modulo $m \in \mathbb{N}$, batch size $n \in \mathbb{N}$, accuracy parameter $\tau$\;
% \If{$y > ng+\tau$}{
%     $z = (y-m)/g$
% }
% \Else{
%     $z = y/g$
% }
% \textbf{Output}: $z$\;
% \end{algorithm}


% and we present a general regret under a particular condition on the $\cP$. These will serve as main building blocks for later sections when we initilize

% \begin{remark}
% A nice feature of Algorithm~\ref{alg:SE} is its flexibility. It provides a generic framework for designing private MAB algorithms under different trust models (central, local and distributed). To see this, one can design a private central MAB algorithm by instantiating $\cR,\cS$ with identity mappings, and $\cA$ with standard DP mechanisms (e.g., Laplace or Gaussian). On the other hand, a private local MAB algorithm is obtained by instantiating $\cR$ with standard DP mechanism and both $\cS$ and $\cA$ with identity mappings\xingyu{$\cA$ is not identity but a sum function}. 
% In fact, we also develop an analytical framework that can be utilized to derive the private regret bounds of Algorithm~\ref{alg:SE} under different trust models in a unified way (see Section~\ref{sec:overview}).
% \end{remark}
% \xingyu{maybe this remark can be removed? My initial thoughts are as follows. 

% 1. Even for continuous noise, Algorithm~\ref{alg:SE} can cover both local and central model with laplace Gaussian noise at different places. This does not need our template protocol $\cP$

% 2. For discrete noise, Algorithm~\ref{alg:SE} AND template protocol $\cP$ can cover both local and central by minor modification of $\cR$, $\cA$.

% 3. For both continous and discrete under three trust models, we provide a unified analytical framework.

% These are three points I want to delivery through this remark.
% }
% \sayak{Can be removed since we have already given remark 4}



% \begin{algorithm}[tb]
%   \caption{Local Randomizer $\cR$}
%   \label{alg:randomizer}
% \begin{algorithmic}[1]
%     \STATE {\bfseries Input:} Each user data $x_i \in [0,1]$
% %   \STATE {\bfseries Parameters:}  precision $g \in \mathbb{N}$, modulo $m \in \mathbb{N}$, batch size $n \in \mathbb{N}$, privacy parameter $\phi$
%   \STATE {\bfseries Parameters:}  precision $g \in \mathbb{N}$, modulo $m \in \mathbb{N}$, batch size $n \in \mathbb{N}$, privacy level $\epsilon$
%   \STATE Encode $x_i$ as $\hat{x}_i = \lfloor{x_i g}\rfloor + \textbf{Ber}(x_ig -\lfloor{x_i g}\rfloor)$
% %   \STATE Generate discrete noise $\eta_i \sim \text{rand}(n,\phi)$ \textcolor{gray}{// a black-box random noise generator}
%     \STATE Generate discrete noise $\eta_i$ (depending on $n,\epsilon,g$) \COMMENT{a black-box random noise generator}
%   \STATE Add noise and modulo clip $y_i = (\hat{x}_i + \eta_i) \Mod m$
%   \STATE {\bfseries Output:} $y_i$ \COMMENT{for secure computation protocol $\cS$}
% \end{algorithmic}
% \end{algorithm}
% \vspace{-2mm}
% \begin{algorithm}[!tb]
%   \caption{Analyzer $\cA$}
% %   \sayak{Can this be written as subroutine of Algo 1? Just to save some space. Also, is it possible to shift the gray texts to far right? I tried but failed...}
% %   }\xingyu{I prefer to keep it as a building block. Let me try to put comments to right}
%   \label{alg:analyzer}
% \begin{algorithmic}[1]
%     \STATE {\bfseries Input:} $\hat{y}$ (output of $\cS$) 
%   \STATE {\bfseries Parameters:}  precision $g \in \mathbb{N}$, modulo $m \in \mathbb{N}$, batch size $n \in \mathbb{N}$, accuracy parameter $\tau \in \Real$
% %   \STATE Let $y \in \mathbb{Z}_m$ be the result of first summing over $\hat{y}$ and then take modulo $m$ 
%   \STATE \textbf{if} $\cS$ is Secure Shuffling \textbf{then}
% \STATE $\quad$ set $y = (\sum \hat{y}) \Mod m  $ \COMMENT{$\hat{y}$ is a set for secure shuffling}
% % \textcolor{gray}{// $\hat{y}$ is a vector for secure shuffling}
% \STATE \textbf{else} set $y = \hat{y}$ \COMMENT{$\hat{y}$ is scalar for secure aggregation} 
% % \textcolor{gray}{// $\hat{y}$ is scalar for secure aggregation}
% %   \IF{$y > ng+\tau$}
% %     \STATE $z = (y-m) / g$ \textcolor{gray}{// correction for underflow}
% %   \ELSE
% %     \STATE $z = y/g$
% %   \ENDIF
% \STATE \textbf{if} $y > ng+\tau$ \textbf{then}
% \STATE $\quad$ set $z = (y-m) / g$ \COMMENT{correction for underflow}
% \STATE \textbf{else} set $z = y/g$
%   \STATE {\bfseries Output:} $z$
% \end{algorithmic}
% \end{algorithm}

\section{Achieving Pure DP in the Distributed Model}
\label{sec:pureDP}
 
% and secure shuffling. 
% All the proofs are in Appendix~\ref{app:pureDP}

% To achieve this, we rely on discrete Laplace noise to guarantee privacy and a careful analysis of random rounding and modular operation to derive the regret bound, which is required to handle the discrete noise. 

% \sayak{Does this algorithm work for variable batch setting? Also, what is the main conceptual difference from Sajed and Shefffet's optimal stopping rule algorithm?}
% \xingyu{This is already variable batch, i.e., double-increasing size. This algorithm is conceptually the same as Sajed's paper, except the added $\cP$. But, I believe the way I present it is more easier to understand and more clean.}
% \sayak{They have some private stopping rule. Right? In our case, we do not have any data-dependent stopping rule.}\xingyu{If you look at their main algorithm, there is no such thing. You can double-check it in case I miss something important:). Or you can regard our algorithm as the same as the shuffle MAB paper with only one important change -- we reset the mean estimate for each batch -- which is also used in Sajed's paper. This will help us to achieve better pure-DP (matching central model) and approximate-DP (i.e., better than shuffle MAB paper by $\sqrt{\log T}$).}\sayak{Question: If I reset mean estimates in the shuffle MAB paper, I would also get the same improvement. Right?}\xingyu{Yes, that's the only difference between ours and the shuffle MAB paper}\sayak{But it won't be pure DP for the shuffle paper?}\xingyu{Sure, it cannot achieve pure DP}\sayak{But shuffle paper can also achieve optimal regret just by doing reset?}\xingyu{it can shave $\sqrt{\log T}$ if they do reset, but it is still not optimal in terms of approximate DP. In fact, the current regret bound under approximate DP in the central model is not clear. I have some question about its bound. }\xingyu{In summary, even the shuffle paper did the reset, because they use standard shuffling protocol, no hope for them to achieve pure DP. The best they can improve is to shave $\sqrt{\log T}$ in its current regret bound if they do reset while attaining approximate DP.}\sayak{I understand the privacy part. We should focus on pure DP in this paper. Else, there will be no significant contribution in the eyes of the reviewers. Else, for approximate DP, what are we gaining from shuffle paper?}

% \xingyu{Pure DP is not enough actually. The material cannot support the whole paper in my opinion. We should consider the following three aspects: privacy, regret, communication. Pure DP is clear. Then, if we move from pure DP, we consider approximate DP, and CDP/RDP. Even in approximate DP, we have some contributions: (1) $\sqrt{\log T}$ (although it is simple). (2) we can handle real reward rather than only binary reward.}

% ****what is the gain from shuffle paper?****
% \xingyu{(1) $\sqrt{\log T}$ (although it is simple). they can also do by reset. (2) we can handle real reward rather than only binary reward. Not consistent with story}

% we should define our goalpost for this paper. I 
% thought we are aiming to match Central pure DP bound and we did that by secagg. Then we can just focus on SecAgg and do all possible things we can do using SecAgg. There should be some common connection between all we do. I am not getting a theme for this paper. Say, we should write about SecAGG as a way of achieveing Distributed DP. That can be a common theme. Then we do Pure DP, approx DP, CDP all and compare with whatever is known in all three sttings like for pure DP compare with Sajed's paper; for approx DP compare with Shuffle MAB paper; for CDP --no comparsion.

% \xingyu{In this way, then you have to argue that SecAgg is better than shuffling? My initial thought is that we just consider SecAgg and Shuffling are just two ways to achieve distributed DP. The theme of this papr is to *investigate how to achieve distributed DP in MAB* no matter which way you use.}

% \sayak{One counterpoint that people might raise that shuffling has been done before. Why are you doing this? Regret is same for both (ignore sqrt(log T)) Exactly, we give a shuffling mechanism for pure DP. So, pure DP part is sorted. That was the point--focus on pure DP. but, your point is that this is not enough. So, in Sec 5.1, you have written shuffling for approx DP. This part is similar (result-wise but not technique-wise) to previous paper (a reviewer will easily argue that they can also save extra factor. Our contribution is only discrete noise). yeah. So, coming to the story now: We can easily sell pure DP part by telling previous work (on dist. DP) have  only considered approximate DP (e.g. shuffle MAB paper). But pure DP better. So, that we get by two diff. procedures. }\xingyu{Yes! This par is clear}

% \sayak{On a side note, I have some questions on exps --will discuss tonight.}\xingyu{sure, np!}\sayak{So, we agree that pure DP is our main selling point? We can then compare with Sajed's paper. They compared with previous paper. If we show our regret matces their, then we are in good shape. Note that Sajed paper's algorithm is differenet than ours. They do not have doubling batch schedule. Instead, they have a differentially private batch schedule (which is elegant). I will go through their paper carefully again}\xingyu{In fact, it is the same. See their line 7 in Alogithm 3. They basically did the same thing.}
% \sayak{But see line 8. At every epoch}\xingyu{instead of using a rough union bound over all T and arms like ours, they use a more refined confidence bound with time and active set, this difference is minor.} \xingyu{You can also compare the two proofs, which basically are the same.}\sayak{I disagree or something I dont understand. There is an $\epsilon$ term in batch schedule in Line 8.}\xingyu{Yes, I agree. But, it seems to me that it is not necessary. In fact, in their proof, they did not use any results established in previous sections. Or I miss something? But, anyway, we first need to make sure that our algorithm is correct:)}


% \xingyu{To sell the second part, we can say: beyond pure DP, the current work only touches approximate DP (of course:)). But, approximate DP has several limitations and moreover the current paper uses a lot of communications. Now, to resolve the limitations of approximate DP and its high communication, we propose use SecAgg with other noise to achieve CDP/RDP}

% \sayak{But, people will ask since you have already achieved pure DP, why are you going for a weaker notion of CDP? Then, we tell that better regret. But is this a good enough story?} \xingyu{because, you can have a slightly better regret in this weaker privacy. or we can sell it like our generic framework is flexible}


% \sayak{One way to do is that--write all about achieveing pure DP etc..-- then tell that oyesss-- general enough framework to capture approx. DP /CDP. But that should come as a by-product of our approch with a mention that it can shave of some log T factor}\xingyu{I will try to finish all the theorems so that we can make the table first.} \sayak{Sec 5.1 might not be needed here. }\xingyu{yes, totally fine, we can put it in appendix anyway}


% \xingyu{Yes! in addition to regret, CDP/RDP is also better than approximate DP}


% \xingyu{I agree, we can put this into later section. They key question here is how to sell CDP/RDP part in a natural way. Currently, I first use approximate DP as a transition so that I can talk about the benefits of CDP/RDP in section 5.2. That's the only reason.}

% \xingyu{But, that is only for approximate DP. We can use shuffle for pure DP. Thus, I think we should also focus on shuffle. For pure DP, I think we are clear: SecAgg and shuffle, done! The remainin part is how to sell CDP/RDP with SecAgg}


% \xingyu{This is for sure. But it is not enough for the paper. This is my opinon. It cannot support the whole story.}

% \subsection{Secure Aggregation}
In this section, we show that Algorithm~\ref{alg:SE} with a specific instantiation of the template protocol $\cP$ is able to achieve pure-DP in the distributed DP model via secure aggregation.\footnote{We show similar results for secure shuffling in Appendix~\ref{app:relaxed-SecAgg}. See also Remark~\ref{rem:relaxed-SecAgg}.}
% We first consider the case when $\cS$ in $\cP$ is implemented via SecAgg. 
As mentioned before, we will treat SecAgg as a black-box function, which implements the following procedure: given $n$ users and their randomized messages $y_i \in \mathbb{Z}_m$ (i.e., integer in $\{0,1,\ldots, m-1\}$) obtained via $\cR$, the SecAgg function $\cS$ faithfully computes the modular sum of the $n$ messages, that is, $\hat{y} = (\sum_{i=1}^{n} y_i) \Mod m$ (i.e., it is perfectly correct), while revealing no further information (e.g., individual message) to a
potential attacker (i.e., it is perfectly secure). % Note that in this case $y = \hat{y}$ in $\cA$  since $\hat{y}$ is already an integer in $\mathbb{Z}_m$.
Now, to guarantee privacy in the distributed model, we need to carefully determine the amount of (discrete) noise in $\cR$ so that the total noise in a batch provides $(\epsilon,0)$-DP. One natural choice is the discrete Laplace noise.

\begin{definition}[Discrete Laplace Distribution]
Let $b > 0$.  A random variable $X$ has a discrete Laplace distribution with scale parameter $b$, denoted by $\textbf{Lap}_{\mathbb{Z}}(b)$, if it has a probability mass function given by
\begin{align*}
    \forall x \in \mathbb{Z}, \quad \prob{X = x} = \frac{e^{1/b} - 1}{e^{1/b} + 1}\cdot e^{-\abs{x}/b}.
\end{align*}
\end{definition}

A key property of discrete Laplace that we will use is its \emph{infinite divisibility}, which allows us to simulate it in a distributed way~\cite[Theorem 5.1]{goryczka2015comprehensive}.

\begin{fact}[Infinite Divisibility of Discrete Laplace]
\label{lem:polya}
A random variable $X$ has a P\'{o}lya distribution with parameters $r \!>\! 0,\beta\!\in\! [0,1]$, denoted by $\textbf{P\'{o}lya}(r,\beta)$, if it has a probability mass function given by
\footnote{ 
% For $r \in \mathbb{N}$, it is essentially defined by counting number of failures $x=0,1,2,\ldots$ in $r+x-1$ trials (last trial is always a success with probability $1-\beta$).
One can sample from $\textbf{P\'{o}lya}$ as follows.
First, sample $\lambda \sim \textbf{Gamma}(r, \beta/(1-\beta))$ and then use it to sample $X \sim \textbf{Poisson}(\lambda)$, which is known to follow $\textbf{P\'{o}lya}(r,\beta)$ distribution \cite{goryczka2015comprehensive}.}
\begin{align*}
    \forall x \in \mathbb{N}, \quad \prob{X = x} = \frac{\Gamma(x+r)}{x!\Gamma(r)}  \beta^x (1-\beta)^r.
\end{align*}
Now, for any $n \in \mathbb{N}$, let $\{\gamma_i^+,\gamma_i^-\}_{i \in [n]}$ be $2n$ i.i.d samples from  $\textbf{P\'{o}lya}(1/n,e^{-1/b})$, then the random variable $\sum_{i=1}^n (\gamma_i^+ - \gamma_i^-)$ is distributed as $\textbf{Lap}_{\mathbb{Z}}(b)$.
\end{fact}

% For any $n \in \mathbb{N}$, let $\{\gamma_i^+,\gamma_i^-\}_{i \in [n]}$ be $2n$ i.i.d samples from the probability distribution $\textbf{P\'{o}lya}(1/n,\beta)$, where 
% a random variable $X$ has a P\'{o}lya distribution with parameters $(r,\beta)$, denoted by $\textbf{P\'{o}lya}(r,\beta)$, if it has a probability mass function given by
% \begin{align*}
%     \forall x \in \mathbb{N}, \quad \prob{X = x} = \frac{\Gamma(x+r)}{x!\Gamma(r)}  \beta^x (1-\beta)^r,
% \end{align*}

% Choose $\beta = e^{-1/b}$, then the random variable $\sum_{i=1}^n \gamma_i^+ - \gamma_i^-$ is distributed as $\textbf{Lap}_{\mathbb{Z}}(b)$, where a random variable $X$ has a P\'{o}lya distribution with parameters $(r,\beta)$, denoted by $\textbf{P\'{o}lya}(r,\beta)$, if it has a probability mass function given by
% \begin{align*}
%     \forall x \in \mathbb{N}, \quad \prob{X = x} = \binom{r+x-1}{r-1}  \beta^x (1-\beta)^r,
% \end{align*}
% where $\binom{r+x-1}{r-1}=\frac{\Gamma(x+r)}{x!\Gamma(r)}$ is defined using Gamma functions (since $r > 0$).\footnote{ For $r \in \mathbb{N}$, it is essentially defined by counting number of failures $x=0,1,2,\ldots$ in $r+x-1$ trials (last trial is always a success with probability $1-\beta$).}


%\begin{remark}[Sampling from P\'{o}lya]
% One can efficiently draw samples from P\'{o}lya distribution. In particular, to draw $X \sim \textbf{P\'{o}lya}(r,\beta)$, one first draw a sample from Gamma distribution, i.e., $\lambda \sim \textbf{Gamma}(r, \beta/(1-\beta))$ and use $\lambda$ to draw $X \sim \textbf{Poisson}(\lambda)$ (see the remark after Theorem 5.1 in~\cite{goryczka2015comprehensive}). Here we use shape and rate parameterization of \textbf{Gamma}.
%\end{remark}


Further, to analyze privacy and regret, we will rely on the following fact on discrete Laplace~\cite{canonne2020discrete}. 
\begin{fact}[Discrete Laplace Mechanism]
\label{lem:disLap_priv_util}
Let $\Delta, \epsilon> 0$. Let $q: \cD^n \to \mathbb{Z}$ satisfy $\abs{q(D) - q(D')} \le \Delta$ for all $D, D'$ differing on a single user's data. Define a mechansim $M: \cD^n \to \mathbb{Z}$ by $M(D) = q(D) + Y$, where $Y \sim \textbf{Lap}_{\mathbb{Z}}(\Delta/\epsilon)$. Then, $M$ satisfies $(\epsilon,0)$-DP. Moreover, for all $m \in \mathbb{N}$,
\begin{align*}
    \prob{Y > m} = \prob{Y <-m} = \frac{e^{-\frac{\epsilon m}{\Delta}}}{e^{\frac{\epsilon}{\Delta}} + 1}.
\end{align*}
\end{fact}

Armed with these facts, we are able to obtain the following main theorem, which shows that the same regret as in the central model is achieved under the distributed model via SecAgg. See Appendix~\ref{app:pureDP} for proof.
\begin{theorem}[Pure-DP via SecAgg]
\label{thm:pure-SecAgg}
Fix any $\epsilon > 0$. Let $\cP = (\cR,\cS,\cA)$ be a protocol such that the noise in $\cR$ (Algorithm~\ref{alg:randomizer}) is given by $\eta_i = \gamma_i^+ - \gamma_i^-$, where $\gamma_i^+,\gamma_i^- \sim^{\text{i.i.d.}} \textbf{P\'{o}lya}(1/n, e^{-\epsilon/g})$, $\cS$ is any SecAgg protocol and $\cA$ is given by Algorithm~\ref{alg:analyzer}. For each batch $b \ge 1$, choose $n = l(b), g = \ceil{\epsilon \sqrt{n}}$, $\tau = \ceil{\frac{g}{\epsilon}\log(2/p)}$, $p =1/T$  and $m = ng + 2\tau + 1$. Then, Algorithm~\ref{alg:SE} instantiated with protocol $\cP$ and confidence radius 
$\beta(b) \!=\! O\!\left(\!\sqrt{\frac{\log(|\Phi(b)|b^2/p)}{2l(b)}}  + \frac{2\log(|\Phi(b)|b^2/p)}{\epsilon l(b)}\!\right)$,
achieves $(\epsilon,0)$-DP in the distributed model. Moreover, it enjoys the expected regret
\begin{align*}
    \ex{\text{Reg}(T)} = O\left(\sum\nolimits_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a} +\frac{K\log T}{\epsilon}\right).
\end{align*}
% Moreover, the communication bits per user before $\cS$ is $O(\log m)$ bits.
\end{theorem}
% Let us now summarize some key implications of this result.

\textbf{Theorem~\ref{thm:pure-SecAgg} achieves optimal regret under pure DP.}
Theorem~\ref{thm:pure-SecAgg} achieves the same regret bound as the one achieved in \cite{sajed2019optimal} under the central trust model with \emph{continuous} Laplace noise. Moreover, it also matches the lower bound obtained under pure DP \cite{shariff2018differentially}, indicating the bound is indeed tight\footnote{With the standard trick of $\Delta_a$, one can directly use Theorem~\ref{thm:pure-SecAgg} to obtain the minimax regret.}. Note that, we achieve this rate under distributed trust model -- a stronger notion of privacy protection than the central model -- while using only discrete privacy noise.



\textbf{Communication bits.}
Algorithm~\ref{alg:SE} needs to communicate $O(\log m)$ bits per user to the secure protocol $\cS$, i.e., communicating bits scales logarithmically with the batch size. In contrast, the number of  communication bits required in existing distributed DP bandit algorithms that work with real-valued rewards (as we consider here) scale polynomially with the batch size~\cite{chowdhury2022shuffle,garcelon2022privacy}. 
% Moreover, modern $\cS$ itself also involves only logarithmic communications~\cite{bell2020secure}.

% \xingyu{shall we add one sentence to say that the communication cost of $\cS$ itself also enjoy logrithmic growth rate, since SecAgg also requires users' additional communication (e.g., masks). Then, refer to appendix.}
% \sayak{cite MAB shuffle paper?}\xingyu{MAB shuffle paper  is a different story. They only deal with binary reward and hence the communication is small (or not that large) actually.}\sayak{can we characterize that?}
% \xingyu{we can, theirs is smaller than ours. so I did not mention that because it is not the same case. I can try to decide our communication for binary case. Otherwise, I prefer not to give it at this place.}\sayak{NEed to write that in the next section. otherwise they will be unhappy. Lets try to complete the picture}ok
% (Note that these work consider shuffling protocol for real-valued rewards ).


% \sayak{ this is a high probability result. Right? Need to state accrdingly with conf sets}\xingyu{This is an expected result, see the definition of regret, which is the same as shuffle MAB paper.}\sayak{But, I need to set $p=1/T$. Setting this makes $\tau$ in the mechanism very large. Why can't we state a high probability result first for any $p$? The same way Sajed's paper does. Then we can set $p=1/T$ and state expected regret. (We can take $p=0.1$ for implementation. ) Is there any roadblock? Also, some people might ask for high prob. bounds.}\xingyu{sure, it is an easy task. But, in MAB, to my best of knowledge, people actually mainly focus on expected regret, see Bubeck's book or other sources. For implementation, we can easily choose any $p$ we like as long as they are consistent. I think the expected regret will be much clear to delivery the key message as in shuffle MAB paper as well as my LDP paper. Finally, even in Sajed's paper, they did not state high probability bound for the regret (only for the number of pulls of sub-optimal arms). The final regret result is still the expected one. }

% \subsection{Secure Shuffling}

\begin{remark}[Pure DP via Secure Shuffling]
\label{rem:relaxed-SecAgg}
It turns out that one can achieve same  privacy and regret guarantees (orderwise) using a \emph{relaxed} SecAgg protocol, which relaxes the SecAgg protocol mentioned above in the following sense: (i) \textbf{relaxed correctness} -- the output of $\cS$ can be used to compute the correct modular sum except at most a small probability (denoted by $\hat{q}$); (ii) \textbf{relaxed security} -- the output of $\cS$ reveals only $\hat{\epsilon}$ more information than the modular sum result. Putting the two aspects together, one obtains a relaxed protocol denoted by $(\hat{\epsilon}, \hat{q})$-SecAgg.
One important benefit of using this relaxation is that it allows us to achieve the same results of Theorem~\ref{thm:pure-SecAgg} via secure shuffling. More specifically, as shown in~\cite{cheu2021pure}, there exists a shuffle protocol that can simulate an $(\hat{\epsilon}, \hat{q})$-SecAgg. Hence, we can directly instantiate $\cS$ using this shuffle protocol to achieve pure DP in the distributed model while obtaining the same regret bound as in the central model. We provide more details on this shuffle protocol in~Appendix~\ref{app:relaxed-SecAgg}, and its performance guarantee in Theorem~\ref{thm:pure-shuffle}.
\end{remark}



% It turns out that a perfect SecAgg is not necessary for the above results. In particular, one can achieve the same privacy guarantee and same order of regret bound  using only a \emph{relaxed} SecAgg as $\cS$, which relaxes a perfect SecAgg above in the following sense: (i) relaxed correctness -- the output of $\cS$ can be used to compute the correct modular sum except at most a small probability (denoted by $\hat{q}$); (ii) relaxed security -- the output of $\cS$ reveals only $\hat{\epsilon}$ more information than the modular sum result. Putting the two aspects together, one obtains a relaxed SecAgg denoted by $(\hat{\epsilon}, \hat{q})$-SecAgg. 
% We provide more details of the relaxed SecAgg in Appendix~\ref{app:relaxed-SecAgg}.

% One important benefit of using a relaxed SecAgg is that it allows us to achieve the same results via secure shuffling. More specifically, as shown in~\cite{cheu2021pure}, there exists a shuffle protocol that can simulate an $(\hat{\epsilon}, \hat{q})$-SecAgg. Hence, we can directly instantiate $\cS$ using this shuffle protocol to achieve pure DP in the distributed model while maintaining the same regret bound as the central model. We provide more intuition on this shuffle protocol in~Appendix~\ref{app:relaxed-SecAgg}, and its performance guarantee in Theorem~\ref{thm:pure-shuffle}.

% In this section, we turn to consider the case when $\cS$ is implemented via a secure shuffling function. The key challenge here is that almost all the existing shuffle protocols can only provides approximate DP when computing the private sum. To overcome this and attain pure DP in the distributed model via shuffling, we will leverage a recent advance in~\cite{cheu2021pure}, which proposes a scheme to simulate a \emph{relaxed} SecAgg using a shuffler along with another local randomizer scheme. By \emph{relaxed} SecAgg, it roughly means that the shuffler's output can be used to compute the correct sum modulo $m$ (as in SecAgg) except at most a  small probability (denoted by $\hat{q}$) and meanwhile reveals only $\hat{\epsilon}$ more information than the modular sum result. 

% To simulate an $(\hat{\epsilon},\hat{q})$-SecAgg via shuffling, the key is to introduce another local randomizer on top of the original $\cR$. More specifically, we let $\cS := S \circ R^n$ in Algorithm~\ref{alg:SE} with $n = l(b)$, $b\ge 1$, where $R$ denotes the additional local randomizer at each user $i \in [n]$ that maps the output of $\cR$ (i.e., $y_i$) into a random binary vector of a particular length $d$. Then, $S$ denotes a standard shuffler that uniformly at random permutes all the received bits from $n$ users (i.e., a total of $n\cdot d$ bits).~\citet{cheu2021pure} has contributed a nice construction of $R$  such that $\cS = S\circ R^n$ can simulate an $(\hat{\epsilon},\hat{q})$-SecAgg for any $\hat{\epsilon}, \hat{q} \in (0,1)$, see more details in Appendix~\ref{app:relaxed-SecAgg}. Finally, note that since the direct output of $\cS$ is a bunch of bits, $y$ in $\cA$ is now the number of ones in the bits modulo $m$.

% To analyze the privacy and regret, we will fully leverage the relaxation property of $(\hat{\epsilon},\hat{q})$-SecAgg so that we can easily adapt our previous results obtained with a perfect SecAgg to this new scenario.

% \begin{theorem}[Pure-DP via Shuffling]
% \label{thm:pure-shuffle}
% Let $\cP_t = (\cR,\cS,\cA)$ be a protocol such that $\cR$ given by Algorithm~\ref{alg:randomizer} injects noise $\eta_i = \gamma_i^+ - \gamma_i^-$, where $\gamma_i^+$ and $\gamma_i^-$ are i.i.d samples from $\textbf{P\'{o}lya}(1/n, e^{-\epsilon/g})$, $\cS$ is an $(\hat{\epsilon},\hat{q})$-SecAgg (e.g., simulated via shuffling),  and $\cA$ is given by Algorithm~\ref{alg:analyzer}. Fix any $\epsilon \in (0,1)$, for each $b \ge 1$, choose $n = l(b), g = \ceil{\epsilon' \sqrt{n}}$, $\tau = \ceil{\frac{g}{\epsilon'}\log(2/p')}$, and $m = ng + 2\tau + 1$, $\hat{\epsilon} = \epsilon/4, \epsilon' = \epsilon/2, \hat{q} = p' = \frac{1}{2T}$. Then, Algorithm~\ref{alg:SE} instantiated with protocol $\cP_t$ is able to achieve $(\epsilon,0)$-DP in the distributed model with expected regret given by 
% \begin{align*}
%     \ex{\text{Reg}(T)} = O\left(\sum_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a} +\frac{K\log T}{\epsilon}\right).
% \end{align*}
% Moreover, the communication per user before $\cS$ is $O(\log m)$ bits.
% \end{theorem}

% \xingyu{One may wonder we can also directly state this general result first and then the perfect SecAgg is a special case. But, I think it is better to first introduce the standard perfect SecAgg and then generalizes it so that people do not have to learn too much at first glance. Also, SecAgg is much easier to understand.}\sayak{Agree. The simpler the presentation, the better.}


\section{Achieving RDP in the Distributed Model}
\label{sec:approx-DP}
% In this section, we aim to show that Algorithm~\ref{alg:SE} can also be instantiated
% with other protocols such that it can achieve privacy guarantees other than pure DP. In such cases, we are often able to achieve a better regret compared to the previous section due to a weaker privacy guarantee. More importantly, when considering approximate DP, Algorithm~\ref{alg:SE} achieves a better regret compared to the state-of-the-art by a factor of $\sqrt{\log T}$. In addition to approximate DP, Algorithm~\ref{alg:SE} can also achieve RDP/CDP, which not only avoids the catastrophic privacy failure in approximate DP, but provides tight privacy accounting for composition. 



% \subsection{SecAgg for CDP and RDP}
% In the last section, we have shown that how to utilize Algorithm~\ref{alg:SE} to improve the state-of-the-art regret bound with shuffling when one aims to achieve approximate DP. However, it also has several limitations. First, approximate DP via binomial noise can have a privacy loss that is infinite with a non-zero probability, leading to catastrophic privacy failures. Second, when one considers privacy composition in MAB\footnote{For example, instead of assuming unique users, one user can participate in multiple rounds during one $T$-round learning process, or she can take part in multiple $T$-round learning processes. In both cases, to calculate the total privacy loss of the repeated user, one needs privacy composition.}, the result via advanced composition theorem can be loose. Third, the shuffle protocol in both~\cite{tenenbaum2021differentially} and Theorem~\ref{thm:approx-shuffle} has a large communication cost per user.

% To resolve the above three limitations \emph{simultaneously}, we will consider the case when $\cS$ is implemented via SecAgg again. Instead of simulating a discrete Lapalce noise in Section~\ref{sec:pureDP}, we will turn to consider two other private noise -- discrete Gaussian and Skellam distribution. These two mechanisms enable us to achieve CDP and RDP, respectively, and both avoid the catastrophic privacy failure. More importantly, both provide a tighter privacy accounting in terms of composition due to moments accountant of the privacy loss random variable. Last, as in Section~\ref{sec:pureDP}, SecAgg enables that each user only sends $O(\log m)$ bits. 


% \subsubsection{Discrete Gaussian Mechanism}
% The discrete Gaussian mechanism is first proposed and investigated by~\cite{canonne2020discrete} and has been recently applied to federated learning~\cite{kairouz2021distributed}. We are the first to apply it to bandit learning. 

% \begin{definition}[Discrete Gaussian Distribution]
% Let $\mu, \sigma \in \Real$ with $\sigma > 0$.  A random variable $X$ has a discrete Gaussian distribution with location $\mu$ and scale $\sigma$, denoted by $\cN_{\mathbb{Z}}(\mu, \sigma^2)$, if it has a probability mass function given by
% \begin{align*}
%     \forall x \in \mathbb{Z}, \quad \prob{X = x} = \frac{e^{-(x-\mu)^2/2\sigma^2}}{\sum_{y \in \mathbb{Z}} e^{-(y-\mu)^2/2\sigma^2} }.
% \end{align*}
% \end{definition}

% The following result from~\cite{canonne2020discrete} will be useful in our privacy and regret analysis.
% \begin{fact}[Discrete Gaussian Privacy and Utility]
% \label{lem:dg-priv-util}
% Let $\Delta, \epsilon> 0$. Let $q: \cX^n \to \mathbb{Z}$ satisfy $\abs{q(x) - q(x')} \le \Delta$ for all $x, x'$ differing on a single entry. Define a randomized algorithm $M: \cX^n \to \mathbb{Z}$ by $M(x) = q(x) + Y$, where $Y \sim \cN_{\mathbb{Z}}(0, \Delta^2/\epsilon^2)$. Then, $M$ satisfies $\frac{1}{2}\epsilon^2$-concentrated differential privacy (CDP). Moreover, $Y$ is $\Delta^2/\epsilon^2$-sub-Gaussian
% and hence
% for all $t \ge 0$,
% \begin{align*}
%     \prob{\abs{Y} \ge t} \le 2 e^{-t^2\epsilon^2/(2\Delta^2)}.
% \end{align*}
% \end{fact}

% However, a direct application of above results does not work. This is because the sum of discrete Gaussian is \emph{not} a discrete Gaussian, and hence one cannot directly apply the privacy guarantee of discrete Gaussian when analyzing the view of the analyzer via summing all the noise from users. To overcome this, we will rely on a recent result in~\cite{kairouz2021distributed}, which shows that under reasonable parameter regimes, the sum of discrete Gaussian is close to a discrete Gaussian. The regret analysis will again build on the generic regret bound for Algorithm~\ref{alg:SE}.

% \begin{theorem}[CDP via SecAgg]
% \label{thm:cdp-SecAgg}
% Let $\cP = (\cR,\cS,\cA)$ be a protocol such that $\cR$ given by Algorithm~\ref{alg:randomizer} injects noise $\eta_i \sim \cN_{\mathbb{Z}}(0,\frac{g^2}{n\epsilon^2})$, $\cS$ is any SecAgg protocol and $\cA$ is given by Algorithm~\ref{alg:analyzer}. Fix $\epsilon \in (0,1)$ and a scaling factor $s \ge 1$, for each $b \ge 1$, choose $n = l(b), g = \ceil{s \epsilon \sqrt{n}}$, $\tau = \ceil{\frac{g}{\epsilon}\sqrt{2\log(2/p)}}$, $p =1/T$  and $m = ng + 2\tau + 1$. Then, Algorithm~\ref{alg:SE} instantiated with protocol $\cP$ is able to achieve $\frac{1}{2}\hat{\epsilon}^2$-CDP with $\hat{\epsilon}$ given by 
% \begin{align*}
%     \hat{\epsilon} \le \min \left\{ \sqrt{ \epsilon^2 + 2\tau  },  \epsilon + \tau \right\},
% \end{align*}
% where $\tau:= 10 \cdot \sum_{k=1}^{\frac{T}{2}-1} e^{-2\pi^2 s^2 \cdot\frac{k}{k+1}}$. Meanwhile, the regret is given by 
% \begin{align*}
%     \text{Reg}(T) = O\left(\sum_{a\in [K]: \Delta >0} \frac{\log T}{\Delta_a} +\frac{K\sqrt{\log T}}{\epsilon}\right),
% \end{align*}
% and the communication messages per user are $O(\log m)$ bits.
% \end{theorem}

% \begin{remark}[Privacy-Communication Trade-off]
% We can observe an interesting trade-off between privacy and communication cost. In particular, as $s$ increases, $\tau$ approaches zero and hence the privacy loss approaches the one under continuous Gaussian. However, a larger $s$ leads to a larger $m$ and hence a larger communication overhead.
% \end{remark}

% \subsubsection{Skellam Mechanism}


% In this section, we will show that beyond pure DP, Algorithm~\ref{alg:SE} along with template protocol $\cP_t$ also offers the possibility to achieve other privacy guarantee that is stronger than approximate DP. In particular, we will show that it can achieve RDP in the distributed model, which not only avoids the catastrophic privacy failure in approximate DP, but provides tight privacy accounting for composition. Further, after the conversion from RDP to approximate DP, the final regret bound could be better than existing regret bound under approximate DP and the one in pure DP established before.
% To achieve this, instead of discrete Laplace in the previous section, we consider another type of discrete noise -- Skellam distribution --  which has recently been applied to the federated learning setting~\cite{agarwal2021skellam} with RDP guarantees. To extend it to the bandit learning setting, a key challenge in the regret analysis is to characterize the tail property of Skellam distribution. This is different from~\cite{agarwal2021skellam} where the variance is sufficient. To this end, we prove that Skellam has sub-exponential tails, which not only is the key to our regret analysis, but also could be of independent interest.



% show that Skellam is a sub-exponential distribution.

% Before that, we first give the definition of Skellam distribution and talk about how to sample from it.


% we will show that one can also apply the recently proposed Skellam mechanism~\cite{agarwal2021skellam} to our generic framework. Compared to discrete Gaussian,  
% Skellam distribution has the advantages that it is closed under summation and enjoys an efficient sampling procedure. Moreover, as shown in~\cite{agarwal2021skellam}, Skellam mechanism is able to achieve RDP and hence it also offers a tight privacy accounting as CDP when analyzing privacy composition. 

% However, a key challenge in the regret analysis is to characterize the tail property of Skellam distribution. This is different from~\cite{agarwal2021skellam} where the variance is sufficient. To this end, we formally show that Skellam is a sub-exponential distribution. 

A natural question to ask is whether one can get a better utility (regret) performance by sacrificing a small amount of privacy. In this section, we show that Algorithm~\ref{alg:SE} along with privacy protocol $\cP$ (Algorithm~\ref{alg:randomizer},\ref{alg:analyzer}) achieves RDP (see Definition~\ref{def:RDP}) in the distributed model. Although RDP is a weaker notion of privacy than pure DP, it avoids catastrophic privacy failure common in approximate DP. It also provides a tighter privacy accounting for composition compared to approximate DP~\cite{mironov2017renyi}.

% advanced composition for approximate DP and the simple composition for pure DP~\cite{mironov2017renyi}.

% \sayak{check}\xingyu{good edits. I have the following thoughts. (1) RDP is better than directly using advanced composition (both yields approximate DP) (2) If one only works in pure DP, then one no longer can use advanced composition (since it only leads to approximate DP). As a result, one can only use simple composition, which grows with $k$ rather than $\sqrt{k}$. How to  state these thoughts without any concerns is a good question. This is because the reviewer may argue, one can also first translate pure DP to RDP, and then apply tight composition. The catch here is that this only gives approximate DP rather than pure DP in the end.}\
% \sayak{Let's just write DP and not worry too much?}\xingyu{I have just added a few words in the last sentence}
% Further, after the conversion from RDP to approximate DP, the final regret bound could be better than existing regret bound under approximate DP and the one in pure DP established before.

To achieve RDP guarantee using discrete noise, instead of discrete Laplace distribution in the previous section, we consider the Skellam distribution --  which has recently been applied in federated learning~\cite{agarwal2021skellam}. In the multi-armed bandit setting, a key challenge in the regret analysis is to characterize the tail property of Skellam distribution. This is different from~\cite{agarwal2021skellam}, where characterizing the variance of Skellam distribution is sufficient. In Proposition~\ref{prop:sk-tail}, we prove that Skellam has sub-exponential tails, which not only is the key to our regret analysis, but also could be of independent interest.

\begin{definition}[Skellam Distribution]
A random variable $X$ has a Skellam distribution with mean $\mu$ and variance $\sigma^2$, denoted by $\textbf{Sk}(\mu,\sigma^2)$, if it has a probability mass function given by 
\begin{align*}
    \forall x \in \mathbb{Z}, \quad \prob{X = x} = e^{-\sigma^2} I_{x-\mu}(\sigma^2),
\end{align*}
where $I_{\nu}(\cdot)$ is the modified Bessel function of the first kind.
\end{definition}

%\begin{remark}
To sample from Skellam distribution, one can rely on existing procedures for  Poisson samples. This is because if $X = N_1 - N_2$, where $N_1, N_2\sim^{\text{i.i.d.}} \textbf{Poisson}(\sigma^2/2)$, then $X$ is $\textbf{Sk}(0,\sigma^2)$ distributed. Moreover, due to this fact, Skellam is closed under summation, i.e., if $X_1 \sim \textbf{Sk}(\mu_1,\sigma_1^2)$ and $X_2 \sim \textbf{Sk}(\mu_2,\sigma_2^2)$, then $X_1 + X_2 \sim \textbf{Sk}(\mu_1 + \mu_2, \sigma_1^2 + \sigma_2^2)$.
%\end{remark}


% We now state the sub-exponential tail property of Skellam. This result is the key to our regret analysis, and it could be of independent interest as well.
\begin{proposition}[Sub-exponential Tail of Skellam]
\label{prop:sk-tail}
Let $X \sim \textbf{Sk}(0,\sigma^2)$. Then, $X$ is $(2\sigma^2,\frac{\sqrt{2}}{2})$-sub-exponential. Hence, for any $p \in (0,1]$, with probability at least $1-p$, 
% $ |X| \le 2\sigma \sqrt{\log(2/p)} + \sqrt{2}\log(2/p).$
\begin{align*}
    |X| \le 2\sigma \sqrt{\log(2/p)} + \sqrt{2}\log(2/p).
\end{align*}
\end{proposition}
With the above result, we can establish the following privacy and regret guarantee of Algorithm~\ref{alg:SE}. See Appendix~\ref{app:approx-DP} for proof.
\begin{theorem}[RDP via SecAgg]
\label{thm:rdp-SecAgg}
Fix any $\epsilon > 0$. Let $\cP = (\cR,\cS,\cA)$ be a protocol such that the noise in $\cR$ (Algorithm~\ref{alg:randomizer}) is given by $\eta_i \sim \textbf{Sk}(0, \frac{g^2}{n\epsilon^2})$, $\cS$ is any SecAgg protocol and $\cA$ is given by Algorithm~\ref{alg:analyzer}. Fix a scaling factor $s \ge 1$. For each batch $b \ge 1$, choose $n = l(b), g = \ceil{s \epsilon \sqrt{n}}$, $\tau = \ceil{\frac{2g}{\epsilon}\sqrt{\log(2/p)} + \sqrt{2}\log(2/p)}$, $p =1/T$  and $m = ng + 2\tau + 1$. Then, Algorithm~\ref{alg:SE} instantiated with protocol $\cP$ and  confidence radius 
$\beta(b) = O\left(\sqrt{\frac{\log(|\Phi(b)|b^2/p)}{2l(b)}}  + \frac{(1+1/s)\log(|\Phi(b)|b^2/p)}{\epsilon l(b)}\right)$, achieves $(\alpha, \hat{\epsilon}(\alpha) )$-RDP in the distributed model for all $\alpha = 2,3,\ldots$, with $\hat{\epsilon}(\alpha)= \frac{\alpha \epsilon^2}{2} + \min\left\{  \frac{(2\alpha -1) \epsilon^2}{4 s^2 }+ \frac{3\epsilon}{2 s^3  }, \frac{3\epsilon^2}{2s}\right\}$.
% $\alpha >1$ and $\alpha \in \mathbb{Z}$ with 
% \begin{align*}
%     \hat{\epsilon}(\alpha)= \frac{\alpha \epsilon^2}{2} + \min\left\{  \frac{(2\alpha -1) \epsilon^2}{4 s^2 }+ \frac{3\epsilon}{2 s^3  }, \frac{3\epsilon^2}{2s}\right\}.
% \end{align*} 
Moreover, it enjoys the regret bound 
\begin{align*}
    \ex{\text{Reg}(T)} = O\left(\sum\nolimits_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a} +\frac{K\sqrt{\log T}}{\epsilon} + \frac{K\log T}{s \epsilon}\right)~.
\end{align*}
% and the communication messages per user are $O(\log m)$ bits.
\end{theorem}
% \begin{theorem}[RDP via SecAgg]
% \label{thm:rdp-SecAgg}
% Fix any $\epsilon > 0$. Let $\cP = (\cR,\cS,\cA)$ be a protocol such that the noise in $\cR$ (Algorithm~\ref{alg:randomizer}) is given by $\eta_i \sim \textbf{Sk}(0, \frac{g^2}{n\epsilon^2})$, $\cS$ is any SecAgg protocol and $\cA$ is given by Algorithm~\ref{alg:analyzer}. Fix a scaling factor $s \ge 1$. For each batch $b \ge 1$, choose $n = l(b), g = \ceil{s \epsilon \sqrt{n}}$, $\tau = \ceil{\frac{2g}{\epsilon}\sqrt{\log(2/p)} + \sqrt{2}\log(2/p)}$, $p =1/T$  and $m = ng + 2\tau + 1$. Then, Algorithm~\ref{alg:SE} instantiated with protocol $\cP$ and  confidence radius 
% $\beta(b) = O\left(\sqrt{\frac{\log(|\Phi(b)|b^2/p)}{2l(b)}}  + \frac{(1+1/s)\log(|\Phi(b)|b^2/p)}{\epsilon l(b)}\right)$, achieves $(\alpha, \hat{\epsilon}(\alpha) )$-RDP in the distributed model for all $\alpha = 2,3,\ldots$, with
% % $\alpha >1$ and $\alpha \in \mathbb{Z}$ with 
% \begin{align*}
%     \hat{\epsilon}(\alpha)= \frac{\alpha \epsilon^2}{2} + \min\left\{  \frac{(2\alpha -1) \epsilon^2}{4 s^2 }+ \frac{3\epsilon}{2 s^3  }, \frac{3\epsilon^2}{2s}\right\}.
% \end{align*} 
% Moreover, it enjoys the regret bound 
% \begin{align*}
%     \ex{\text{Reg}(T)} = O\left(\sum\nolimits_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a} +\frac{K\sqrt{\log T}}{\epsilon} + \frac{K\log T}{s \epsilon}\right)~.
% \end{align*}
% % and the communication messages per user are $O(\log m)$ bits.
% \end{theorem}

% Now, we summarize implications of this result.
\textbf{Privacy-Regret-Communication Trade-off.}
Observe that the scaling factor $s$ allows us to achieve different trade-offs. If $s$ increases, both privacy and regret performances improve. In fact, for a sufficiently large value of $s$, the third term in the regret bound becomes sufficiently small, and we obtain an improved regret bound compared to Theorem~\ref{thm:pure-SecAgg}. Moreover,
the RDP privacy guarantee improves to $\hat \epsilon(\alpha)\approx \frac{\alpha\epsilon^2}{2}$, which is the standard RDP rate for Gaussian mechanism~\cite{mironov2017renyi}. However, a larger $s$ leads to an increase of communicating bits per user, but only grows logarithmically, since Algorithm~\ref{alg:SE} needs to communicate $O(\log m)$ bits to the secure protocol $\cS$. 

\textbf{RDP to Approximate DP.}
To shed more insight on Theorem~\ref{thm:rdp-SecAgg}, we convert our RDP guarantee to approximate DP for a sufficiently large $s$. It holds that under the setup of Theorem~\ref{thm:rdp-SecAgg}, for sufficiently large $s$, one can achieve $(O(\epsilon),\delta)$-DP with regret $O\big(\sum_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a} +\frac{K\sqrt{\log T\log(1/\delta)}}{\epsilon}\big)$ (via Lemma~\ref{applem:conversion}). The implication of this conversion is three-fold. \textbf{First}, this regret bound is $O(\sqrt{\log T})$ factor tighter than that achieved by \cite{tenenbaum2021differentially} using a shuffle protocol with same $(\epsilon,\delta)$-DP guarantee.
 \textbf{Second}, it yields a better regret performance compared to the bound achieved under $(\epsilon,0)$-DP in Theorem~\ref{thm:pure-SecAgg} when the privacy budget $\delta > 1/T$. This observation is consistent with the fact that a weaker privacy guarantee typically warrants a better utility bound. \textbf{Third}, this conversion via RDP also yields a gain of $O(\sqrt{\log(1/\delta)})$ in the regret when dealing with privacy composition (e.g., when participating users across different batches are \textit{not unique}) compared to~\cite{tenenbaum2021differentially} that can only rely on approximate DP (see Appendix~\ref{app:return} for details). This results from the fact that RDP provides a tighter composition compared to approximate DP.

% \sayak{gain compared to what? Shuffle-MAb? This point can be removed}\xingyu{Yes, shuffle MAB. Privacy accounting for composition is one motivation for RDP, and hence we better keep it.}



% In this case, by the conversion lemma (Lemma~\ref{applem:conversion} in Appendix~\ref{app:CDP}), we have that Algorithm~\ref{alg:SE} with Skellam noise also guarantees $(O(\epsilon\sqrt{\log(1/\delta)}),\delta)$-DP. Thus, under the $(O(\epsilon),\delta)$-DP guarantee, the additional cost in the expected regret is mainly $O\left(\frac{K\sqrt{\log T \log(1/\delta)}}{\epsilon}\right)$. 

% This is strictly better than existing approximate-DP regret bound in the distributed model~\cite{tenenbaum2021differentially} by a $O(\sqrt{\log T})$ factor and also yields a gain compared to the stronger pure-DP when $\log(1/\delta) < \log(T)$. This conversion via RDP will also yields a gain of $O(\sqrt{\log(1/\delta)})$ in the regret when dealing with privacy composition for returning users (see Appendix~\ref{app:return}).






\begin{remark}[Achieving RDP with discrete Gaussian]
As shown in~\cite{canonne2020discrete}, one can also achieve RDP guarantee using discrete Gaussian noise. In this work, we consider Skellam distribution since it is closed under summation and enjoys efficient sampling procedure as opposed to discrete Gaussian \cite{agarwal2021skellam}. Nevertheless, as a proof of flexibility of our proposed framework, we show in Appendix~\ref{app:CDP} that Algorithm~\ref{alg:SE} with discrete Gaussian noise can guarantee RDP with a similar regret bound. 
%obtained under Skellam noise.
\end{remark}

% We end this section by remarking that one may consider using discrete Gaussian~\cite{canonne2020discrete} instead of Skellam. As argued in~\cite{agarwal2021skellam}, Skellam has the advantages of being closed under summation and enjoying efficient sampling procedure compared to discrete Gaussian. Nevertheless, as a proof of the flexibility of our proposed algorithm and protocol, we also show that our algorithm with discrete Gaussian noise can guarantee RDP with a similar regret gain (see Appendix~\ref{app:CDP}). 
% Furthermore, we discuss the gain of a tighter privacy accounting of RDP in MAB for composition in Section~\ref{sec:conclusion}.



\section{Key Techniques: Overview}
\label{sec:overview}
In this section, we provide an overview of the key techniques behind the privacy guarantees and regret bounds in previous sections. In fact, we will show that the results of Theorem~\ref{thm:pure-SecAgg} and \ref{thm:rdp-SecAgg} can be obtained via a clean generic analytical framework, which not only covers the analysis of distributed pure DP/RDP via both SecAgg and shuffling, but also offers a unified view of private MAB under central, local and distributed DP models. 

As in many private learning algorithms, the key is to characterize the impact of added privacy noise on the utility. In our case, this reduces to capturing the tail behavior of total noise (i.e., the term $n_a(b):= R_a(b) - \sum_{i=1}^{l(b)}r_a^i(b)$) added at each batch $b$ for each active arm $a$ by the privacy protocol $\cP$.  The following lemma gives a generic regret bound under mild tail assumptions on $n_a(b)$. See Appendix~\ref{app:proofLem1} for proof.
\begin{lemma}[Generic regret under tail bound on total noise]
\label{lem:general-regret-informal}
For any $p \in (0,1]$, let there exist constants $\sigma, h > 0$ such that for all $b\ge 1$, $a \in [K]$, it holds that $|n_a(b)| \le \cN:=O\left(\sigma \sqrt{\log(KT/p)} + h\log(KT/p)\right)$, with probability at least $1-p$. Then, running Algorithm~\ref{alg:SE} with $p=1/T$ and confidence width $\beta(b) = O\left(\sqrt{\log(KT/p)/l(b)} + \cN/l(b)\right)$ at batch $b$, we acieve the expected regret
\begin{align*}
    \ex{\text{Reg}(T)} = O\Big(\sum\nolimits_{a\in [K]: \Delta_a >0} \frac{\log T}{\Delta_a} + K\sigma \sqrt{\log T} + K h {\log T}\Big).
\end{align*}
\end{lemma}
An acute reader may notice that the bound $\cN$ on the noise is the tail bound for a sub-exponential distribution and it reduces to the bound for sub-Gaussian tail if $h = 0$. Moreover, our SecAgg protocol $\cP$ with discrete Laplace noise (as given in Theorem~\ref{thm:pure-SecAgg}) satisfy this bound with $\sigma=\sqrt{2}/\epsilon, h=1/\epsilon$. Similarly, our protocol with Skellam noise (as given in Theorem~\ref{thm:rdp-SecAgg}) satisfy this bound with $\sigma=O(1/\epsilon), h=1/(s\epsilon)$. Therefore, we can build on the above general result to directly obtain our regret bounds (Theorem~\ref{thm:pure-SecAgg},\ref{thm:rdp-SecAgg}). In the following, we will highlight the high-level idea behind our privacy and regret analysis in the distributed DP model. 
% Then, we highlight the key differences in each specific secure protocols. 

\textbf{Privacy.} For distributed DP, by definition, the view of the server during the entire algorithm needs to be private. Since each user only contributes once\footnote{This assumption that users only contributes once is adopted in nearly all previous works for privacy analysis in bandits. 
We also provide a privacy analysis for returning users via RDP, see Appendix~\ref{app:return}.
}, by the parallel-composition of DP, it suffices to ensure that the each view $\hat{y}_a(b)$ is private. To this end, under both SecAgg and shuffling,  the distribution of $\hat{y}_a(b)$ can be simulated via $(\sum_{i} y_i) \Mod m$, which can be further reduced to $\left(\sum_i \hat{x}_i + \eta_i\right) \Mod m$ by the distributive property of modular sum. Now, we consider a  mechanism $\cH$ that accepts an input dataset $\{\hat{x}_i\}_i$ and outputs $\sum_i \hat{x}_i + \sum_i \eta_i$. By post-processing, it suffices to show that $\cH$ satisfies pure DP or RDP. To this end, the variance $\sigma_{tot}^2$ of the total noise $\sum_i \eta_i$ needs to scale with the sensitivity of $\sum_i \hat{x}_i$. Thus, each user within a batch only needs to add a proper noise with variance of $\sigma_{tot}^2/n$.
Finally, by the particular distribution properties of the noise, one can show that $\cH$ is pure DP or RDP, and hence, obtain the privacy guarantees. 

\textbf{Regret.} Thanks to Lemma~\ref{lem:general-regret-informal}, we only need to focus on the tail of $n_a(b)$. To this end, fix any batch $b$ and arm $a$. We have $\hat{y}= \hat{y}_a(b)$, $x_i = r_a^i(b)$, $n = l(b)$ for $\cP$ and we need to establish that with probability at least $1-p$, for some $\sigma$ and $h$,
\begin{align}
\label{eq:goal-int}
    \abs{\cA(\hat{y}) - \sum\nolimits_i x_i} \le O\left(\sigma \sqrt{\log(1/p)} + h \log (1/p)\right).
\end{align}

To get the bound, inspired by~\cite{balle2020private,cheu2021pure}, we divide the LHS into $\text{Term (i)} \!=\! \abs{\cA(\hat{y}) -  \sum_i \hat{x}_i/g}$ and $\text{Term (ii)} \!=\! \abs{ \sum_i \hat{x}_i/g - \sum_i x_i}$,
% \begin{align*}
%     \abs{\cA(\hat{y}) - \sum\nolimits_i x_i} \le \underbrace{\abs{\cA(\hat{y}) -  \sum\nolimits_i \hat{x}_i/g}}_{\text{Term (i)}} + \underbrace{\abs{ \sum\nolimits_i \hat{x}_i/g - \sum\nolimits_i x_i}}_{\text{Term (ii)}},
% \end{align*}
where $\text{Term (i)}$ captures the error due to privacy noise, modular operation and possible relaxed correctness in secure shuffling, while Term (ii) captures the error due to random rounding. In particular, Term (ii) can be easily bounded via sub-Gaussian tail since the noise is bounded. Term (i) needs care for the possible underflow due to modular operation by considering two different cases (see the second \emph{if-else} clause in Algorithm~\ref{alg:analyzer}). In both cases, one can show that Term (i) is upper bounded by $\tau /g$ with high probability, where $\tau$ is the tail bound on the total privacy noise $\sum_i \eta_i$. Thus, depending on particular privacy noise and parameter choices, one can find $\sigma$ and $h$ such that~\eqref{eq:goal-int} holds, and  hence, obtain the corresponding regret bound by Lemma~\ref{lem:general-regret-informal}.

% To get the bound, inspired by~\cite{balle2020private,cheu2021pure}, we divide the LHS into two terms as follows. 
% \begin{align*}
%     \abs{\cA(\hat{y}) - \sum\nolimits_i x_i} \le \underbrace{\abs{\cA(\hat{y}) -  \sum\nolimits_i \hat{x}_i/g}}_{\text{Term (i)}} + \underbrace{\abs{ \sum\nolimits_i \hat{x}_i/g - \sum\nolimits_i x_i}}_{\text{Term (ii)}},
% \end{align*}
% where $\text{Term (i)}$ captures the error due to private noise, modular operation and possible approximate correctness in secure shuffling, while Term (ii) captures the error due to random rounding. In particular, Term (ii) can be easily bounded via sub-Gaussian tail since the noise is bounded. Term (i) needs care for the possible underflow due to modular operation by considering two different cases. In both cases, one can show that Term (i) is upper bounded by $\tau /g$ with high probability, where $\tau$ is the tail bound on the total noise $\sum_i \eta_i$. Thus, depending on particular private noise and parameter choices, one can find $\sigma$ and $h$ such that~\eqref{eq:goal-int} holds, hence the corresponding regret bound by Lemma~\ref{lem:general-regret-informal}.

% In addition to above general techniques, we highlight some key technical details in establishing each theorem. 
% For Theorem~\ref{thm:pure-SecAgg}, we utilize the infinite divisibility of discrete Laplace via {P\'{o}lya} distribution. For Theorem~\ref{thm:rdp-SecAgg}, the key is to establish the first tight concentration bound on Skellam distribution.

% In addition to this, Theorem~\ref{thm:pure-shuffle} also requires a careful analysis of the relaxed secure shuffling, i.e., relaxed security and correctness.  

\begin{remark}
As a by-product of our generic analysis technique, Algorithm~\ref{alg:SE} and privacy protocol $\cP$ along with Lemma~\ref{lem:general-regret-informal} provide a new and structured way to design and analyze private MAB algorithms under central and local models with discrete private noise (see Appendix~\ref{app:central-local} for details). This enables us to reap the benefits of working with discrete noise (e.g., finite-computer representations, bit communications) in all three trust models (central, local and distributed).
\end{remark}

% \begin{align*}
%     \hat{\epsilon}(\alpha) \le \frac{\alpha \epsilon^2}{2} + \min\left\{\frac{(2\alpha - 1) \epsilon^4}{4 g^2} + \frac{3\epsilon^4}{2g^3}, \frac{3\epsilon^2}{2g}\right\}.
% \end{align*}
% Meanwhile, the regret is given by 
% \begin{align*}
%     \text{Reg}(T) = O\left(\sum_{a\in [K]: \Delta >0} \frac{\log T}{\Delta_a} +\frac{K\sqrt{\log T} }{\epsilon} + K \log T\right).
% \end{align*}
% Moreover, the communication per user is $O(\log m)$.





% \subsection{Shuffling for Approximate DP}
% \xingyu{we can remove this section to appendix}

% We first consider the case when $\cS$ is implemented via a shuffler. In this case, we make the following two improvements over the existing work that attains $(\epsilon,\delta)$-DP via shuffling~\cite{tenenbaum2021differentially}: (i) our regret bound shaves $\sqrt{\log T}$ from the one in~\cite{tenenbaum2021differentially}; (ii) our regret and privacy guarantees hold for non-binary reward whereas~\cite{tenenbaum2021differentially} only considers binary rewards.

% The improvements are achieved through the following two key components. First, although Algorithm~\ref{alg:SE} is also a successive elimination algorithm as in~\cite{tenenbaum2021differentially}, one key difference is that the mean estimate is reset at the beginning of each batch. Since the batch size is exponentially increasing, this resetting allows us to get rid of the concentration of sum of sub-Gaussian noise (hence an $\sqrt{\log T}$ improvement) while only paying a cost of constant factor in the regret. Second, we build upon the very recent advance in shuffle protocol for scalar sum~\cite{cheu2021shuffle}, which is capable of handling real number. 

% In the following, we briefly describe the shuffle protocol in~\cite{cheu2021shuffle} for computing the sum $\sum_{i \in [n]}x_i$ where $x_i \in [0,1]$ (i.e., Algorithm 1 in~\cite{cheu2021shuffle}). We denote it by $\hat{\cP} = (\hat{\cR}, \hat{\cS}, \hat{\cA})$ where $\hat{\cS}$ is a standard shuffler. The local randomizer $\hat{\cR}$ at each user first applies the random rounding and then inject  binomial noise for privacy. In particular, as in Algorithm~\ref{alg:analyzer}, it encodes the input $x_i \in [0,1]$ by $\hat{x}_i = \lfloor{x_i g}\rfloor + \textbf{Ber}(x_ig -\lfloor{x_i g}\rfloor)$. Then, it generates binomial noise for privacy, $\eta_i \sim \textbf{Bin}(b,p)$ where $b \in \mathbb{N}, p \in (0,1)$ control the privacy. The output of $\hat{\cR}$ is collection of $g+b$ bits such that the sum equals $\hat{x}_i + \eta_i$. The shuffler $\hat{\cS}$ simply permutes all the bits (i.e., $n\cdot (g+b)$). The analyzer $\hat{\cA}$ sums all the bits and remove the bias due to rounding and noise, i.e., output $z = \frac{1}{g}(\sum_{i=1}^{(g+b)n}y_i - pbn)$. 

% \begin{theorem}[Approximate DP via Shuffling]
% \label{thm:approx-shuffle}
% Let $\hat{\cP} = (\hat{\cR}, \hat{\cS}, \hat{\cA})$  be the shuffle protocol given by~\cite[Algorithm 1]{cheu2021shuffle}. For each $b\ge 1$, choose $n = l(b), g = \ceil{2\sqrt{n}}, b > \frac{720 g^2 \log(2/\delta)}{\epsilon^2 n}, p = \frac{360 g^2 \log(2/\delta)}{b \epsilon^2 n}$.
% Then, Algorithm~\ref{alg:SE} instantiated with protocol $\hat{\cP}$ is able to achieve $(\epsilon,\delta)$-DP  in the distributed model for any $\epsilon \le 15, \delta \in (0,1/2)$ with regret given by 
% \begin{align*}
%     \text{Reg}(T) = O\left(\sum_{a\in [K]: \Delta >0} \frac{\log T}{\Delta_a} +\frac{K\sqrt{\log T \log(1/\delta)}  }{\epsilon}\right).
% \end{align*}
% \end{theorem}
% \xingyu{Caution here: Although the above regret removes $\sqrt{\log T}$ compared to last section, it also introduces an additional $\sqrt{\log(1/\delta)}$. For *meaningful* choice of $\delta$, i.e., $\delta \le 1/T$, this new regret bound has the same order as before. Thus, we need be careful when we say it has a better regret bound than the pure-DP case. }

% % \section{Achieving Distributed DP via Shuffling}

% % \section{Achieving Central and Local DP via Discrete Noise}

\section{Simulation Results}\label{sec:sim}

% \xingyu{It is not suitable to justify our gap by simply saying that we are considering a weaker trust model. We might say something more in depth like: we have another layer of noise in our confidence bound due to data quantization (so that one can use discrete noise and SecAgg), which will lead to a slightly larger confidence, which further leads to a slight gap in the empirical performance. }

% \xingyu{Some observations:
% \begin{itemize}
%     \item For $K=10$, easy, the results are nicer:) 
%     \item For small $\eps$, RDP gain is obvious. 
%     \item In fact, the batch schedule needs not be $2^b$, basically $a^b$ where $a \ge  2$ is fine. Sajed's paper basically use $a = 4$ (of course, there is another term depending on $\epsilon$, ignore it). Maybe, I can update the algorithm by replacing $2$ by $a$. This will allows us to choose a better $a$.\sayak{Sajed is also $2^b$. Got it one part $4^b$. I think that is the reason they get better than us.}
%     \item I use $a = 8$, which is good. 
%     \item But, let's first see your results, then we can decide whether or not need any updates. These are fine:) Just run it aside.  \sayak{Currently I am running with $2^b$ and old conf width. Once you update Lemma 2, i can run with new stuff}
% \end{itemize}
% }


% \sayak{Summary of findings: schedule of arm elimination depends heavily on the constants hidden in the confidence sets. Need to find some principled way. Sajed's algorithm is performing much better, i.e., discarding sub-optimal arms much earlier than ours.}\xingyu{I have updated the confidence bound, see Appendix.}


\begin{figure}[t]
		\begin{subfigure}[t]{.32\linewidth}
			\includegraphics[width = 2.2in]{Figures/Gauss-easy-new-10-very-low.pdf}
			\vskip -2mm
			\caption{$\epsilon=0.1, K =10$}
		\end{subfigure}\ \
		\begin{subfigure}[t]{.32\linewidth}
			\includegraphics[width = 2.2in]{Figures/Gauss-easy-new-10-low.pdf}
			\vskip -2mm
			\caption{$\epsilon=0.5,K=10$}
		\end{subfigure}\ \
		\begin{subfigure}[t]{.34\linewidth}
			\includegraphics[width = 2.2in]{Figures/Gauss-hard-new-10-very-low.pdf}
			\vskip -2mm
			\caption{$\epsilon=0.1,K=10$}
		\end{subfigure}
		\vskip -2mm
		\caption{\footnotesize{Comparison of time-average regret for Dist-DP-SE, Dist-RDP-SE, and DP-SE in Gaussian bandit instances under (a, b) large reward gap (easy instance) and (c) small reward gap (hard instance). 
% 		In all cases, regret of Dist-DP-SE and Dist-RDP-SE matches the regret of DP-SE.
}  }
\label{fig:all_algos}
%\xingyu{I still prefer to only plot y-axis from 0 to $0.04$ for (c)?

		\vspace{-5mm}
\end{figure}

In this section, we empirically evaluate the regret performance of our successive elimination scheme with SecAgg protocol (Algorithm~\ref{alg:SE}) under distributed trust model, which
we abbreviate as Dist-DP-SE and Dist-RDP-SE when the randomizer $\cR$ is instantiated with P\'{o}lya noise (achieves pure DP) and Skellam noise (achieves RDP), respectively. We compare them with the DP-SE algorithm of \cite{sajed2019optimal} that works only with \emph{continuous} Laplace noise and achieves optimal regret under pure DP in the central model. We fix confidence level $p = 0.1$ and study comparative performances under varying privacy levels $\epsilon < 1$.  Similar to \cite{vaswani2020old}, we consider easy and hard MAB instances: in the former, arm means are sampled uniformly in $[0.25, 0.75]$,
while in the latter, those are sampled in $[0.45, 0.55]$. We consider real rewards -- sampled from Gaussian distribution with aforementioned means and projected to $[0,1]$.
We plot time-average regret $\text{Reg}(T)/T$ in Figure~\ref{fig:all_algos} by averaging results over 20 randomly generated bandit instances.
% We consider both discrete, binary rewards sampled from Bernoulli distributions, as well as continuous rewards
% sampled from beta distributions.
We observe that as $T$ becomes large, the regret performance of Dist-DP-SE matches the regret of DP-SE. The slight gap in small $T$ regime is the cost that we pay to achieve distributed privacy using discrete noise without access to a trusted server (for higher $\epsilon$ value, this gap is even smaller). In addition, we find that a relatively small scaling factor ($s=10$) provides a considerable gain in regret under RDP compared to pure DP, especially when $\epsilon$ is small (i.e., when the cost of privacy is not dominated by the non-private part of regret).
The experimental findings are consistent with our theoretical results. Here, we note that our simulations are proof-of-concept only and we did not tune any hyperparameters.
More details and additional plots are given in Appendix~\ref{app:exps}.

% arises possibly due to data quantization needed in Dist-DP-SE, which introduces some error in regret.




% we have another layer of noise in our confidence bound due to data quantization (so that one can use discrete noise and SecAgg), which will lead to a slightly larger confidence, which further leads to a slight gap in the empirical performance.



% In addition, we find that a relatively small scaling factor $s$ provides a gain for Dist-RDP-SE compared to Dist-DP-SE when $\epsilon$ is small. The experimental findings are consistent with our theoretical results. More details can are given in Appendix~\ref{app:exps}.

% \xingyu{here is the concern, people may say RDP should be better than DP-SE}. 

% \xingyu{another reason why RDP gain is not obvious is due to the fact of our choices of problem instances. The gap is at most $0.5$, which means that the non-private term already dominates the regret, the additive privacy term is small for $\epsilon > 0.5$}
% In addition, we find that a higher value of scale $s$ achieves a lower regret for Dist-RDP-SE.
% a larger regret than LinUCB-JDP. Moreover, the regret performance of LinUCB-SDP (in fact for any private


% \xingyu{I am still a little bit uncomfortable with the gap. The reason is that it might cause reviewers to question our results. I know we need to tune the crs parameter, but our message here is not to beat Sajed. Rather, we are able to match their results with the tuning of the crs parameter, I think it is fine. As a backup, I am running crs = 0.5 for our algorithms and all the other parameters are the same.  }

% \sayak{Graphs are updated.}
% \xingyu{sure, I am just running for backup:)}great yeah sometimes like that sometime crs=0.1 much worse though (never converge) I actually got some graphs that matches upload it today.be careful
% \xingyu{really? great!!!! In the worst case, we can show one figure in appendix to show that after a small tuning, we can match in pure DP and RDP is better than Sajed. Then, that's enough.}
% \xingyu{crs = 0.5 is not ok, since ours would be better than Sajed as you have observed..hahha hhahha let me do it for crs = 0.8. In the worst case, we can show one figure in appendix to show that after a tuning }

% \xingyu{if there still exists a gap, then we can explicitly say that we did not tune any parameters:)}








% \begin{figure}[t]
% 		\begin{subfigure}[t]{.3\linewidth}
% 			\includegraphics[width = 1.75in]{Figures/Gauss-easy-new-10-very-low.pdf}
% 			\caption{$\epsilon=0.1$, easy}
% 		\end{subfigure}\ \
% 		\begin{subfigure}[t]{.3\linewidth}
% 			\includegraphics[width = 1.75in]{Figures/Gauss-easy-new-10-low.pdf}
% 			\caption{$\epsilon=0.5$, easy}
% 		\end{subfigure}\ \
% 		\begin{subfigure}[t]{.3\linewidth}
% 			\includegraphics[width = 1.75in]{Figures/Gauss-easy-new-10-very-high.pdf}
% 			\caption{$\epsilon=10$, easy}
% 		\end{subfigure}\\
% 		\begin{subfigure}[t]{.3\linewidth}
% 			\includegraphics[width = 1.75in]{Figures/Gauss-hard-new-10-very-low.pdf}
% 			\caption{$\epsilon=0.1$, hard}
% 		\end{subfigure}\ \
% 		\begin{subfigure}[t]{.3\linewidth}
% 			\includegraphics[width = 1.75in]{Figures/Gauss-hard-new-10-high.pdf}
% 			\caption{$\epsilon=5$, hard}
% 		\end{subfigure}\ \
% 		\begin{subfigure}[t]{.3\linewidth}
% 			\includegraphics[width = 1.75in]{Figures/Gauss-easy-SE-10-low.pdf}
% 			\caption{$\epsilon=0.5$, easy}
% 		\end{subfigure}\\
% 		 \vspace{0mm}
% 		\caption{\footnotesize{Comparison of time-average regret for Dist-DP-SE, Dist-RDP-SE, and DP-SE with privacy level $\epsilon=0.1$ under Gaussian bandit instances with (a) small gap (easy) and (b) large gap (hard). In all cases, regret of Dist-DP-SE and Dist-RDP-SE matches the regret of DP-SE.}  }\label{fig:all_algos}
% 		\vspace{0mm}
% \end{figure}
% \xingyu{For (d) and (e), we might only plot y-axis above zero? (f) is for easy? the same as (b)? it looks different}\sayak{yes, same as b but with batch schedule $2^b$. PLotting is what it generated.}\xingyu{got it, but for (d) and (e), we might only plot positive part since the regret is always positive?}\sayak{Now, we need to discuss what to keep. RDP with different scalings are not visible much. Some graphs co-incide etc. Need to find a better way to present.}\xingyu{for smaller $\epsilon$, it still has some gain over pure DP (but the gain is not obvious from 10 to 100 is also fine, which tells that 10 is enough), which aligns with theory since for larger $\epsilon$, the term is already a smaller term?. The key thing we want to say is that $s > 1$ yields gain compared to pure DP, which basically $s=1$. Whether or not we have much gain from 10 to 100 is a second thing.}

% \xingyu{or we can tune a little bit and plot addition ones in appendix where RDP has a obvious gain compared to Sajed? Then, we will emphasize in the main part that we directly use the derived confidence interval without tuning. After May.19, we can add more results in appendix (with tuning)}
% \xingyu{Bern is not necessary I think for this paper, since data quantization only leads to noise for real-valued reward.}

% \xingyu{It appears to me that the gap is still large between pure DP case. I will try to specify the constants in our method to test a little bit.} \sayak{Sure. Gap is explainable.We have a much better trust model than central model. Order wise behavior is similar. }\xingyu{All is about a tight confidence. Divide $4$ in the first term of the confidence bound is sufficient, which is justified by Hoffeding inequality. Currently, our code did not divide it by any constant. See my email:)}


% \xingyu{Yes, but I think our algorithm is kind of weaker. If we only consider the non-private one, ours is also worse, am I right? Their batch size is larger than ours}\xingyu{we can also change our SE algorithm to theirs, but only add $\cP$. }

\section{Conclusion}\label{sec:conclusion}
We show that MAB under distributed trust model can achieve pure DP while maintaining the same regret under central model. In addition, RDP is also achieved in MAB udner distributed trust model for the first time. Both results are obtained via a unified algorithm design and performance analysis. More importantly, our work also opens the door to a promising research direction -- private online learning with distributed DP guarantees, including contextual bandits and reinforcement learning. 
% general, about privacy in multi-armed bandits.

% \sayak{Please add couple of lines}\xingyu{shall we just summary the key contributions? since we only have three-four lines maybe}
% To illustrate this, let us consider a simplified music app that uses MAB algorithm to recommend music to its users. Suppose a Latin girl named Alice recently downloads the app and likes many Latin music. To illustrate this, let us consider a simplified music app that uses MAB algorithm to recommend music to its users. Suppose a Latin girl named Alice recently downloads the app and likes many Latin %music. To illustrate this, let us consider %a simplified music app that uses MAB 
% algorithm to recommend music to its users. Suppose a Latin girl named Alice recently downloads the app and likes many Latin music. 
% \xingyu{now we have enough space I think. Also, check the checklist:)}\sayak{Thanks. I think we need a broader impact section also}
% \xingyu{within 9 pages?}\sayak{No. outside}

% \paragraph{Returning users} see Appendix~\ref{app:return}

% \paragraph{Achieving CDP } see Appendix~\ref{app:CDP}

% \paragraph{UCB algorithm} see Appendix~\ref{app:UCB} 
% \xingyu{In fact, for pure DP, UCB algorithm can indeed achieve optimal regret with a careful concentration. That is, sum of sub-exponential does not hurt since the number of noise is smaller than $\log(T)$, i.e., the number of batches (see Lemma~\ref{lem:sum-subexp}). But, for sum of sub-Gaussian, it will hurt the  theoretical performance compared to our resetting to zero, i.e, additional $\sqrt{\log T}$ factor due to accumulated noise. Could you please take a look to double-check this? }

